A survey of parameterized algorithms and the complexity of edge modification

The survey provides an overview of the developing area of parameterized algorithms for graph modification problems. We concentrate on edge modification problems, where the task is to change a small number of adjacencies in a graph in order to satisfy some required property.

==> abstract.tex <==

\begin{abstract}
  \noindent
  %
  This survey contains an in-depth history and overview of the parameterized and
  kernelization complexity of graph modification problems.  We consider a vast
  area of modification problems, including vertex deletions, edge deletions,
  completions, and editing, as well as some contraction related problems.
  
  \medpause
  % 
  The main focus is on edge modification problems such as edge deletion,
  completion and editing.
\end{abstract}


==> contractions.tex <==
 %!TEX root =survey.tex
\clearpage
\section{Edge contractions}\label{sec:contr}
In this section we consider  the operation of edge contraction. 
 For a family of graphs $\cal F$, the  problem where the only allowed edit operation is edge contraction, is called {\sc$\cal  F$-Contraction}. For a graph $G$ and an edge $e=uv\in E(G)$, {\em contraction} of an edge $uv$ in $G$ results in a graph $G/e$, which is obtained by deleting $u$ and $v$ from $G$, adding a new vertex $w_e$ and making $w_e$ adjacent to the neighbors of $u$ or $v$ (other than $u,v$). A graph $G$ is \emph{contractible} to a graph $H$, if there exists a subset $X\subseteq E(G)$, such that if we contract each edge from $X$, then the resulting graph is isomorphic to $H$. For several families of
graphs $\cal F$, early papers by Watanabe et al.~\cite{watanabe81,watanabe1983np} and Asano and Hirata~\cite{asano1983edge} showed that {\sc $\cal F$-Contraction} is \np-hard. The \np-hardness of problems like {\sc Tree Contraction} and {\sc Path Contraction}, which are the {\sc $\cal F$-Contraction} problems for the family of trees and paths, respectively, follows easily from~\cite{asano1983edge,brouwer1987contractibility}.


Heggernes at al.\cite{tree-contraction}  show that {\sc Tree Contraction}  is solvable in
$4^k n^{\cO(1)}$ time by polynomial-space algorithm, as well as by a deterministic $4.98^k n^{\cO(1)} $ time algorithm. However, {\sc Tree Contraction} admits no polynomial kernel unless  \ph.
 {\sc Path Contraction} is solvable in time 
 $2^{k+o(k)} +n^{\cO(1)} $ and admits  a kernel with at most $5k + 3$ vertices.


{\sc Bipartite Contraction}, contracting to a bipartite graph,  is  known to be \fpt  \cite{HeggernesHLP13}. The double-exponential running time from \cite{HeggernesHLP13} was improved to $2^{\cO(k^2)}\cdot n^{\cO(1)} $ by 
 Guillemot  and Marx \cite{guillemot2013faster}. Contracting to planar graph was shown to be \fpt by Golovach, van 't Hof and  Paulusma 
 \cite{GolovachHP13}.
\textsc{Split Contraction}, contracting to a split graph was shown to be \fpt by Guo and Cai \cite{guo2015obtaining}.   \textsc{Split Contraction} admits no polynomial kernel unless \ph.
 

 
 

The \emph{Hadwiger number} $h(G)$ of a  graph $G$ is  the largest number $h$ for which the complete graph $K_h$ is a minor of $G$. Equivalently, $h(G)$ is 
the maximum  size of the largest complete graph that can be obtained from $G$  by contracting edges. It is named after Hugo Hadwiger, who conjectured    in 1943 
that the Hadwiger number of $G$ is always at least as large as its  chromatic number.
According to Bollob\'{a}s,   Catlin, and Erd\H{o}s, this conjecture remains  ``one of the deepest unsolved problems in graph theory'' \cite{MR593989}.
 
 
The Hadwiger number of an $n$-vertex graph $G$ can be easily computed in time $n^{\cO(n)}$ by  brute-forcing through all possible partitions  of the vertex set of $G$ into connected sets, contracting each set into one vertex and checking whether the resulting graph is a complete graph.  
% The question whether 
%the Hadwiger  number of a graph can be computed in   single-exponential  $2^{\cO(n)}$ time 
%was asked explicitly in  \cite{agrawal2017split,DBLP:journals/jacm/CyganFGKMPS17,LingasW09}. 
%Our main result  provides a negative answer to this   long-standing open question. 
On the other hand, \todo{add reference} 
unless the Exponential Time Hypohtesis (ETH) is false, there does not exist an algorithm computing the Hadwiger number of an $n$-vertex graph in time $n^{o(n)}$.


 A restricted version of \textsc{Path Contraction}, is the problem \textsc{$P_t$-Contraction}, where $t$ is a fixed constant. \textsc{$P_t$-Contraction} is shown to be \np-hard even for $t=4$, while for $t\leq 3$, the problem is polynomial time solvable~\cite{brouwer1987contractibility}. \textsc{$P_t$-Contraction} alone had received lot of attention for smaller values of $t$, even when the input graph is from a very structured family of graphs (for instance, see ~\cite{brouwer1987contractibility,van2009partitioning,HeggernesHLP14,dabrowski2017contracting,fiala2013note,kern2018contracting}, and the references therein). 
 For \textsc{$P_t$-Contraction} 
an algorithm of running time $(2-\varepsilon_t)^n$ for some $\varepsilon_t>0$ depending from $t$  was given in  \cite{agrawal_et_al:LIPIcs:2019:10587}.





 



==> editparam.tex <==

\newcommand\cur[1]{\ensuremath{{\cal{#1}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Edit distance as paramater for other problems (Christophe)}\label{sec:editparam}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this section, we report results on problems different from edge modification problems that are parameterized by an edit distance and on edge modification problems that are parameterized by an edit distance that is not the distance to the target class.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Treewidth and Minimum Fill-in parameterized by the distance to split graphs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\cite{Man10} shows that Treewidth and Minimum Fill-In are FPT for almost split graphs, more precisely for the so called split$+ke$ graphs, which are these graphs that can be turned into a split graph by deleting at most $k$ edges. The parameter used in the FPT algorithm is precisely the upperbound $k$ on the distance to split graphs. \cite{Man10} design an $O(2^{k\log k})$ algorithm for both problems. The technique involves the enumeration in FPT time of all minimal chordal completions of the graph.

This is an example of a FPT algorithm that is parameterized by the distance to some class of graphs (here split graphs) but where the aim of the problem is to compute something else than this distance. In the case of \cite{Man10}, the aim is either to compute the distance to another (very related) class of graphs, Minimum Fill-in, or another parameter that quantify the complexity of the graph, Treewidth. Note that the target class in the Minimum Fill-in problem is chordal graphs, which is a superclass of split graphs. In addition, note that computing the treewidth is closely related to chordal graph completion: the difference being that the quantity to minimize is not the number of edges added but instead the maximum clique size of the completed graph. Finally, it is worth noting that both Minimum Fill-in and Treewidth are polynomially computable on split graphs. Then the result of \cite{Man10} can be understood as taking advantage of the proximity of the input graph with a class $\cur{C}$ where these two parameters are easy to compute in order to compute it in FPT time parameterized by the distance to $\cur{C}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Boxicity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In \cite{ABC12b,ABC12}, the problem considered is to compute the boxicity of a graph, which is a graph parameter quantifying the difficulty of encoding a graph with a certain encoding scheme (namely as intersections of boxes in a d-dimensional space). This parameter is not related to edge modification problem. \cite{ABC12b,ABC12} show a nice general result: for any family $\cur{F}$ of bounded boxicity, taking as parameter the number $k=k_1+k_2$ of edge modifications in order to obtain a graph in $\cur{F}$, that is $G\in \cur{F}+k_1 e-k_2 e$, they design an $O(2^{k^2\log k})$ FPT approximation algorithm (with a small additive constant) for computing the boxicity of $G$. This gives as a particular case, the same result using as a parameter edit distances such as interval edge completion, proper interval edge deletion, planar edge deletion. They are also able to retrieve results that are not parameterized by edge edit distances, such as the results in~\cite{ACS10} that are parameterized by Minimum Vertex Cover, Feedback Vertex Set, Max Leaf Number (maximum number possible of leaves in a spanning tree of the graph).

Again, these results can be understood as using the proximity with a class $\cur{C}$ having a good behaviour with regard to the considered problem, here having bounded boxicity, in order to extend this nice behaviour in a parameterized way to graphs that almost belong to $\cur{C}$, taking as a parameter the edit distance to $\cur{C}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Coloring}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As mentionned earlier, the results presented in Section~\ref{sec:editparam} so far can be seen as extending the good behaviour of a class of graphs $\cur{C}$ with regard to some problem to the graphs that are almost in $\cur{C}$, via an algorithm parameterized by the distance to $\cur{C}$. The best example of this general approach is provided by the coloring problem on almost chordal graphs.

\cite{Cai03} shows that given a modulator of the graph (i.e. a set of modifications to be performed in order to reach the target class), a graph $G$ in $\cur{F}-ke$, where $\cur{F}$ is closed under edge contraction and admits a polynomial time algorithm to compute an optimal coloring, an optimal coloring of $G$ can be found in FPT time. This implies, since the problem of finding a modulator of a chordal$-ke$ graph is FPT, that coloring a chordal$-ke$ graph is FPT, even without a modulator given a priori.
A similar result is shown for $\cur{F}+ke$ if the chromatic polynomial can be computed in polynomial time on $\cur{F}$, which is not the case for chordal graphs. Finally, \cite{Cai03} shows that $split+k_1e-k_2e$ with $k_1+k_2\leq k$ can also be colored in FPT time.


In~\cite{Mar06}, these results are completed in the following manner: it is shown that coloring is FPT on chordal+ke graphs, that is graphs where there exist at most $k$ edges whose deletion results in a chordal graph. Again, the modulator, i.e. the edges to be removed, are supposed given as part of the output. Nevertheless, this supposition is not a limitation since it was shown later that finding such a set of edges is FPT~\cite{Mar10,cao2014chordal}. The algorithm of~\cite{Mar06} uses a dynamic programming scheme along the rooted clique tree of the underlying chordal graph, where the additional edges are considered. The clique tree has been previously transformed into a nice tree where each node is binary and corresponds to only one of the three following operations: join, loss of a vertex, gain of a vertex. Moreover, the graph is modified so that additional edges are pairwise non-incident. Two colorings of the children of one node can then be combined iff these two colorings don't assign the same color to the two vertices incident to one additional edge (called special vertex). This is encoded in each node by keeping the list of all possible colorings, described only by a set of couples encoding which color is assigned to each special vertex. Thus, two colorings are compatible iff the set of couples describing them are disjoint. The main tool to get a FPT algorithm is to reduce the size of the list of colorings which is kept in each node. As we are only interested in checking whether there exists another set (from the other node) which is disjoint with one set of this node, and since all the sets have size at most $2k$, then it is possible to keep a list of representative sets of length at most $2^{4k} poly(n)$, with the property that the existence of such a disjoint couple of sets is equivalent to the same existence in the original list. In addition, these representative lists can be composed together to get the representative list of the parent of two nodes. Therefore the dynamic programming scheme along the tree, from the leaves to the root, is shown to be FPT in $k$.



==> former-tables.tex <==

\newpage

\subsection{Former tables}


\begin{table}[tp]
  \centering%
  \renewcommand{\arraystretch}{1.25}%
  \rowcolors{3}{}{gray!20}%
  \begin{tabular}{*4l}
    \toprule
    & \multicolumn{3}{c}{Problem} \\
    \cmidrule(lr){2-4}
    %
    Graph class &  \pname{Deletion}   &  \pname{Completion}  &  \pname{Editing} \\
    % 
    \midrule
    % 
    Bipartite
    & \FPT~\cite{guo2006compressionbased} % EDGE DEL
    & \pt % EDGE COMPL
    & see deletion % EDGE EDIT
    \\
    Perfect
    & open~\cite{heggernes2013parameterized} % EDGE DEL
    & open % EDGE COMPL
    & open % EDGE EDIT
    \\
    Planar
    & \FPT~\cite{kawarabayashi2007computing}
    (minor closed~\cite{adler2008computing,robertson1994graph})% EDGE DEL
    & \pt % EDGE COMPL
    & see deletion % EDGE EDIT
    \\
    Chordal
    & see editing % EDGE DEL
    & \SUBEPT~\cite{fomin2013subexponential} % EDGE COMPL
    & \FPT~\cite{cao2014chordal} % EDGE EDIT
    \\
    Interval
    & open % EDGE DEL
    & \SUBEPT~\cite{bliznets2016subexponential} % EDGE COMPL
    & open % EDGE EDIT
    \\
    Proper Interval
    & \FPT~\cite{cao2016linear} % EDGE DEL
    & \SUBEPT~\cite{bliznets2015subexponential} % EDGE COMPL
    & open % EDGE EDIT
    \\
    Comparability
    & open % EDGE DEL
    & open % EDGE COMPL
    & open % EDGE EDIT
    \\
    Permutation
    & see completion % EDGE DEL
    & open % EDGE COMPL
    & open % EDGE EDIT
    \\
    Circular arc
    & open % EDGE DEL
    & open % EDGE COMPL
    & open % EDGE EDIT % NP-c see burzyn
    \\
    Distance-hereditary
    & \FPT % EDGE DEL
    & \FPT % EDGE COMPL
    & \FPT % EDGE EDIT
    \\
    Wheel-free
    & \wtwo~\cite{lokshtanov2008wheelfree} % EDGE DEL
    & open % EDGE COMPL
    & open % EDGE EDIT
    \\
    $4$-leaf power
    & see editing % EDGE DEL
    & see editing % EDGE COMPL
    & \FPT~\cite{dom2005extending, dom2008closest} % EDGE EDIT
    \\
    $t$-leaf power
    & open % EDGE DEL
    & open % EDGE COMPL
    & open % EDGE EDIT
    \\
    \bottomrule%
    \multicolumn{4}{c}{\textbf{Fixed-parameter tractability}} \\
  \end{tabular}
  \caption{
    Summary of some FPT (or lack thereof) results.
  }
  \label{tab:fpt-results}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "survey"
%%% End:



\begin{table}[tp]
  \centering%
  \renewcommand{\arraystretch}{1.25}%
  \rowcolors{3}{}{gray!20}%
  \begin{tabular}{*4l}
    \toprule
    & \multicolumn{3}{c}{Problem} \\
    \cmidrule(lr){2-4}
    %
    Graph class &  \pname{Deletion}   &  \pname{Completion}  &  \pname{Editing} \\
    % 
    \midrule
    % 
    \KW
    & no~\cite{kratsch2013two} % EDGE DEL
    & not studied % EDGE COMPL
    & no~\cite{kratsch2013two} % EDGE EDIT
    \\
    $3$-Leaf Powers
    & see editing % EDGE DEL
    & see editing % EDGE COMPL
    & $k^3$~\cite{bessy2010polynomial} % EDGE EDIT
    \\
    $4$-Leaf Powers
    & open?todo % EDGE DEL
    & open?todo % EDGE COMPL
    & open?todo % EDGE EDIT
    \\
    Bicluster
    & see editing % EDGE DEL
    & \pt % EDGE COMPL
    & $6k$~\cite{guo2008improvedbicluster} % EDGE EDIT
    \\
    Bipartite
    & $k^{3}$~\cite{kratsch2014compression}$^\dagger$ % EDGE DEL
    & \pt % EDGE COMPL
    & \pt % EDGE EDIT
    \\
    Chain
    & see editing % EDGE DEL
    & see editing % EDGE COMPL
    & $k^2$~\cite{drange2015threshold} % EDGE EDIT
    \\
    Chordal
    & open % EDGE DEL
    & $k^2$~\cite{natanzon2000polynomial} % EDGE COMPL
    & open % EDGE EDIT
    \\
    Claw-free
    & open % EDGE DEL
    & open? % EDGE COMPL
    & open? % EDGE EDIT
    \\
    $2$-Club Cluster
    & open % EDGE DEL
    & ? % EDGE COMPL
    & ? % EDGE EDIT
    \\
    Cluster
    & see editing % EDGE DEL
    & \pt % EDGE COMPL
    & $2k$~\cite{chen2012kernel} % EDGE EDIT
    \\
    Cograph
    & see editing % EDGE DEL
    & see editing % EDGE COMPL
    & $k^3$~\cite{guillemot2013nonexistence} % EDGE EDIT
    \\
    Diamond
    & $k^3$~\cite{sandeep2015parameterized} % EDGE DEL
    & todo % EDGE COMPL
    & todo % EDGE EDIT
    \\
    Grid
    & see editing % EDGE DEL
    & see editing % EDGE COMPL
    & $k^4$~\cite{diaz2006fast} % EDGE EDIT
    \\
    Interval
    & open % EDGE DEL
    & open % EDGE COMPL
    & open % EDGE EDIT
    \\
    Linear forest
    & $9k$~\cite{feng2014randomized} % EDGE DEL
    & \pt % EDGE COMPL
    & see deletion % EDGE EDIT
    \\
    Planar
    & open % EDGE DEL
    & \pt % EDGE COMPL
    & see deletion % EDGE EDIT
    \\
    $s$-Plex Cluster
    & see editing (TODO?) % EDGE DEL
    & see editing % EDGE COMPL
    & $s^2k$~\cite{guo2010more} % EDGE EDIT
    \\
    Proper Interval
    & todo % EDGE DEL
    & $k^3$~\cite{bessy2013polynomial} % EDGE COMPL
    & todo % EDGE EDIT
    \\
    Split
    & $k^2$~\cite{ghosh2015faster} % EDGE DEL
    & see deletion % EDGE COMPL
    & \pt~\cite{hammer1981splittance} % EDGE EDIT
    \\
    Threshold
    & see editing % EDGE DEL
    & see editing % EDGE COMPL
    & $k^2$~\cite{drange2015threshold} % EDGE EDIT
    \\
    Triangle-free
    & $6k$~\cite{brugmann2009generating} % EDGE DEL
    & \pt % EDGE COMPL
    & see deletion % EDGE EDIT
    \\
    Trivially Perfect
    & $k^7$~\cite{drange2015polynomial} % EDGE DEL
    & $k^2$~\cite{guo2007problem} % EDGE COMPL
    & see deletion  % EDGE EDIT
    \\
    $P_\ell$-free, $\ell > 4$
    & no~\cite{cai2012polynomial} % EDGE DEL
    & see deletion % EDGE COMPL
    & see deletion  % EDGE EDIT
    \\
    $C_\ell$-free, $\ell > 3$
    & no~\cite{cai2012polynomial} % EDGE DEL
    & see deletion % EDGE COMPL
    & see deletion  % EDGE EDIT
    \\
    \bottomrule
    \multicolumn{4}{c}{Polynomial kernel} \\
  \end{tabular}
  \caption{
    Summary of some kernelization results.  The kernel sizes are
    to be interpreted as having $O(\;\cdot\;)$ number of vertices, unless in the
    linear cases, where a specific constant is given.
    %
    The negative result is under the assumption that \noph.  $^\dagger$~means a
    \corp{} kernel, and the size is the number of bits in the representation up
    to a polylogarithmic factor.
    %
    \FPT{} denotes the problem is known to be fixed-parameter tractable, thereby
    admitting an exponential kernel.
  }
  \label{tab:kernel-results}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "survey"
%%% End:



\begin{table}[tp]
  \centering%
  \renewcommand{\arraystretch}{1.25}%
  \rowcolors{3}{}{gray!20}%
  \begin{tabular}{*4l}
    \toprule
    & \multicolumn{3}{c}{Problem} \\
    \cmidrule(lr){2-4}
    %
    Graph class &  \pname{Deletion}   &  \pname{Completion}  &  \pname{Editing} \\
    % 
    \midrule
    % 
    $C_4$-free
    & \cclass{ETH}  % EDGE DEL
    & \cclass{ETH} % EDGE COMPL
    & open  % EDGE EDIT
    \\
    Chain                 
    & see completion % EDGE DEL
    & \csq~\cite{drange2015exploring} % EDGE COMPL
    & \csq~\cite{drange2015threshold} % EDGE EDIT
    \\
    Cograph         
    & see completion % EDGE DEL
    & \cclass{ETH}~\cite{drange2015exploring}  % EDGE COMPL
    & \cclass{ETH}~\cite{drange2015polynomial} % EDGE EDIT
    \\
    \pname{Fast}$^\dagger$
    & \csq~\cite{alon2009fast} % EDGE DEL
    & \pt  % EDGE COMPL
    & see deletion % EDGE EDIT
    \\
    Interval
    & open? % EDGE DEL
    & \csq~\cite{bliznets2016subexponential}  % EDGE COMPL
    & open? % EDGE EDIT
    \\
    Trivially Perfect     
    & \cclass{ETH}~\cite{drange2015exploring}  % EDGE DEL
    & \csq~\cite{drange2015exploring} % EDGE COMPL
    & \cclass{ETH}~\cite{drange2015polynomial}   % EDGE EDIT
    \\
    Threshold
    & see completion % EDGE DEL
    & \csq~\cite{drange2015exploring}  % EDGE COMPL
    & \csq~\cite{drange2015threshold}  % EDGE EDIT
    \\
    Split
    & $2^{O(\sqrt k)}$~\cite[Exercise~5.17]{cygan2015parameterized} % EDGE DEL
    & see deletion % EDGE COMPL
    & \pt~\cite{hammer1981splittance} % EDGE EDIT
    \\
    % 
    $P_4$-free
    & see completion % EDGE DEL
    & \cclass{ETH}~\cite{drange2015exploring} % EDGE COMPL
    & \cclass{ETH}~\cite{drange2015polynomial} % EDGE EDIT
    \\
    Pseudosplit
    & $2^{O(\sqrt k)}$~\cite{cygan2015parameterized, drange2015exploring}  % EDGE DEL
    & see deletion % EDGE COMPL
    & \pt % EDGE EDIT
    \\
    Proper Interval
    & open? % EDGE DEL
    & $c^{k^{2/3} \log k}$~\cite{bliznets2015subexponential}  % EDGE COMPL
    & open? % EDGE EDIT
    \\
    \begin{tabular}[c]{@{}l@{}} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BICLUSTER
      Bicluster \\
      $p$-Bicluster
    \end{tabular} % BICL + p-BIC
    & 
    \begin{tabular}[c]{@{}l@{}}
      see editing \\
      see editing
    \end{tabular} % EDGE DEL
    & 
    \begin{tabular}[c]{@{}l@{}}
      \pt \\
      \pt
    \end{tabular} % EDGE COMPL
    & 
    \begin{tabular}[c]{@{}l@{}}
      \cclass{ETH} \\
      $c^{p \sqrt k \log(pk)}$
    \end{tabular} % EDGE EDIT
    \\
    \begin{tabular}[c]{@{}l@{}} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CLUSTER
      Cluster \\
      $p$-Cluster
    \end{tabular} % CL + p-C
    & 
    \begin{tabular}[c]{@{}l@{}}
      see editing \\
      see editing
    \end{tabular} % EDGE DEL
    & 
    \begin{tabular}[c]{@{}l@{}}
      \pt \\
      \pt
    \end{tabular} % EDGE COMPL
    & 
    \begin{tabular}[c]{@{}l@{}}
      \cclass{ETH} \\
      $2^{\sqrt{pk}}$~\cite{fomin2014tight}
    \end{tabular} % EDGE EDIT
    \\
    % \begin{tabular}[c]{@{}l@{}} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CLUB CLUSTER
    %   TODO CLUB \\
    %   TODO $d$-Club $p$-Cluster
    % \end{tabular} % CL + p-C
    % & 
    % \begin{tabular}[c]{@{}l@{}}
    %   todo \\
    %   todo
    % \end{tabular} % EDGE DEL
    % & 
    % \begin{tabular}[c]{@{}l@{}}
    %   todo \\
    %   todo
    % \end{tabular} % EDGE COMPL
    % & 
    % \begin{tabular}[c]{@{}l@{}}
    %   todo \\
    %   todo~\cite{misra2013subexponential}
    % \end{tabular} % EDGE EDIT
    % \\
    \begin{tabular}[c]{@{}l@{}} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STARFOREST
      Starforest \\
      $p$-Starforest
    \end{tabular}
    &
    \begin{tabular}[c]{@{}l@{}}
      \cclass{ETH} \\
      see editing
    \end{tabular} % EDGE DEL
    &
    \begin{tabular}[c]{@{}l@{}}
      \pt \\
      \pt
    \end{tabular}
     % EDGE COMPL
    &
    \begin{tabular}[c]{@{}l@{}}
      \cclass{ETH}\\
      $2^{3\sqrt{pk}}$
    \end{tabular} % EDGE EDIT
    \\
    \bottomrule
  \end{tabular}
  \caption{
    Summary of some subexponentiality results.  All the running
    times should be taken as $\Ostar(\;\cdot\;)$.  \cclass{ETH} means that the
    problem is \npci, and that there is
    no $2^{o(k)}\poly(n)$ algorithm  under the assumption of the exponential
    time hypothesis.
  }
  \label{tab:subept-results}
\end{table}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "survey"
%%% End:


%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\normalsize
\centering
%\begin{tabular}{|c|| >{\centering}m{2cm} | >{\centering}m{2cm} || >{\centering}m{2cm} | >{\centering}m{2cm} || >{\centering}m{2cm} | >{\centering}m{2cm} |}
\hspace*{-2.4cm}\begin{tabular}{| >{\centering}m{2.8cm} || >{\centering}m{2.8cm} | >{\centering}m{2.8cm} || >{\centering}m{2.8cm} | >{\centering}m{2.8cm} || >{\centering}m{2.8cm} | >{\centering}m{2.8cm} |}
\hline
$\curs{F}$-free class & \multicolumn{2}{c||}{completion} & \multicolumn{2}{c||}{deletion} & \multicolumn{2}{c|}{edition} \tabularnewline
\hline
\hline
$\set{2K_2,C_5,K_3}$ (chain) & KER~$k^2$~\cite{bessy2013polynomial,drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{fomin2013subexponential,drange2015threshold} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^2$~\cite{guo2007problem,drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold} & KER~$k^2$~\cite{drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold} \tabularnewline
\hline
$\set{2K_2,C_4,P_4}$ \textbf{*} (threshold) & KER~$k^2$~\cite{drange2015threshold} KER~$k^3$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold,drange2015exploring} ~~NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^2$~\cite{drange2015threshold} KER~$k^3$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold,drange2015exploring} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^2$~\cite{drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold} \tabularnewline
\hline
$\set{C_4,P_4}$ (trivially perfect) & KER~$k^3$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015exploring} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^7$~\cite{DP17} & FPT~$2.45^k$~\cite{NG12} NOSUB~\cite{drange2015exploring} & KER~$k^7$~\cite{DP17} & NOSUB~\cite{DP17} \tabularnewline
\hline
$\set{2K_2,C_4,C_5}$ \textbf{*} (split) & KER~$k^2$~\cite{ghosh2015faster} KER~$k^4$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{ghosh2015faster} & KER~$k^2$~\cite{ghosh2015faster} KER~$k^4$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{ghosh2015faster} & - & - \tabularnewline
\hline
$\set{2K_2,C_4}$ \textbf{*} (pseudosplit) & - & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015exploring} & - & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015exploring} & - & - \tabularnewline
\hline
\hline
$\set{claw, diamond}$ & - & - & KER~$k^{24}$~\cite{CPP+17} & NOSUB~\cite{CPP+17} & - & - \tabularnewline
\hline
$\set{K_{1,s}, K_t}_{s>1,t>2}$ & - & - & KER~\cite{ASS17} & - & - & - \tabularnewline
\hline
\end{tabular}
\medskip
\caption{Parameterized complexity of some edge modification problems into $\curs{F}$-free graph classes, with $\curs{F}$ a finite family of graphs. For each kind of problem (completion, deletion or editing), the left column reports results on polynomial kernels and the right one reports results on the complexity of FPT algorithms. A star next to the name of the class marks autocomplemented classes, for which any result for one of the completion problem or deletion problem automatically gives the same result for the other problem.\label{tab:F-free}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\normalsize
\centering
%\begin{tabular}{|c|| >{\centering}m{2cm} | >{\centering}m{2cm} || >{\centering}m{2cm} | >{\centering}m{2cm} || >{\centering}m{2cm} | >{\centering}m{2cm} |}
\hspace*{-1.3cm}\begin{tabular}{| >{\centering}m{1.8cm} || >{\centering}m{2.6cm} | >{\centering}m{2.6cm} || >{\centering}m{2.6cm} | >{\centering}m{2.6cm} || >{\centering}m{2.6cm} | >{\centering}m{2.6cm} |}
\hline
$H$-free class & \multicolumn{2}{c||}{completion} & \multicolumn{2}{c||}{deletion} & \multicolumn{2}{c|}{edition} \tabularnewline
\hline
\hline
$K_3$ & \multicolumn{2}{c||}{undefined} & KER~$k^3$~\cite{brugmann2009generating} & - & \multicolumn{2}{c|}{not meaningful} \tabularnewline
\hline
$K_4$ & \multicolumn{2}{c||}{undefined} & $k^4$~\cite{cai2012polynomial} & NOSUB~\cite{ASS17b} & \multicolumn{2}{c|}{not meaningful} \tabularnewline
\hline
$P_3$ ~~(cluster) & \multicolumn{2}{c||}{polynomial} & KER~$k^3$~\cite{GGH+05} & FPT~$1.41^k$~\cite{BD11} FPT~$1.77^k$~\cite{GGH+05} NOSUB~\cite{bessy2010polynomial} & KER~$2k$~\cite{chen2012kernel,CC12} KER~$4k$~\cite{Guo09} KER~$6k$~\cite{fellows2007efficient} KER~$k^3$~\cite{GGH+05} & FPT~$1.76^k$~\cite{BD11} FPT~$2.27^k$~\cite{GGH+05} NOSUB~\cite{bessy2010polynomial} \tabularnewline
\hline
$P_4$ (cograph) & $k^3$~\cite{guillemot2013nonexistence} & NOSUB~\cite{drange2015exploring} & $k^3$~\cite{guillemot2013nonexistence} & NOSUB~\cite{drange2015exploring} & $k^3$~\cite{guillemot2013nonexistence} & NOSUB~\cite{DP17} \tabularnewline
\hline
diamond & \multicolumn{2}{c||}{polynomial} & $k^3$~\cite{sandeep2015parameterized,CRS+18} $k^4$~\cite{FGK+11} & NOSUB~\cite{sandeep2015parameterized,ASS17b} & $k^8$~\cite{CRS+18} & NOSUB~\cite{ASS17b} \tabularnewline
\hline
claw & - & NOSUB~\cite{ASS17b} & - & NOSUB~\cite{ASS17b} & - & NOSUB~\cite{ASS17b} \tabularnewline
\hline
paw & - & NOSUB~\cite{ASS17b} & - & NOSUB~\cite{ASS17b} & - & NOSUB~\cite{ASS17b} \tabularnewline
\hline
$C_4$ & NOKER~\cite{guillemot2013nonexistence} & NOSUB~\cite{drange2015exploring} & NOKER~\cite{guillemot2013nonexistence} & NOSUB~\cite{drange2015exploring} & NOKER~\cite{guillemot2013nonexistence} & NOSUB~\cite{ASS17b} \tabularnewline
\hline
\end{tabular}
\medskip
\caption{Parameterized complexity of edge modification problems into $H$-free graph classes, with $H$ a graph on three or four vertices. Note that the complements of these graphs are not listed as both completion and deletion problems are considered.\label{tab:H-free}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\normalsize
\centering

%\begin{center}
\hspace*{-2cm}\begin{tabular}{| >{\centering}m{2cm} || >{\centering}m{2.8cm} | >{\centering}m{2.8cm} || >{\centering}m{2.8cm} | >{\centering}m{2.8cm} || >{\centering}m{2.8cm} | >{\centering}m{2.8cm} |}
\hline
graph class & \multicolumn{2}{c||}{completion} & \multicolumn{2}{c||}{deletion} & \multicolumn{2}{c|}{edition} \tabularnewline
\hline
\hline
chain & KER~$k^2$~\cite{bessy2013polynomial,drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{fomin2013subexponential,drange2015threshold} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^2$~\cite{guo2007problem,drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold} & KER~$k^2$~\cite{drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold} \tabularnewline
\hline
\hline
3-leaf power & KER~$k^3$~\cite{bessy2010polynomial} & - & KER~$k^3$~\cite{bessy2010polynomial} & - & KER~$k^3$~\cite{bessy2010polynomial} & - \tabularnewline
\hline
\hline
cluster & \multicolumn{2}{c||}{polynomial} & KER~$k^3$~\cite{GGH+05} & FPT~$1.41^k$~\cite{BD11} FPT~$1.77^k$~\cite{GGH+05} NOSUB~\cite{bessy2010polynomial} & KER~$2k$~\cite{chen2012kernel,CC12} KER~$4k$~\cite{Guo09} KER~$6k$~\cite{fellows2007efficient} KER~$k^3$~\cite{GGH+05} & FPT~$1.76^k$~\cite{BD11} FPT~$2.27^k$~\cite{GGH+05} NOSUB~\cite{bessy2010polynomial} \tabularnewline
\hline
threshold \textbf{*} & KER~$k^2$~\cite{drange2015threshold} KER~$k^3$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold,drange2015exploring} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^2$~\cite{drange2015threshold} KER~$k^3$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold,drange2015exploring} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^2$~\cite{drange2015threshold} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015threshold} \tabularnewline
\hline
trivially perfect & KER~$k^3$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015exploring} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & KER~$k^7$~\cite{DP17} & FPT~$2.45^k$~\cite{NG12} NOSUB~\cite{drange2015exploring} & KER~$k^7$~\cite{DP17} & NOSUB~\cite{DP17} \tabularnewline
\hline
cograph \textbf{*} & KER~$k^3$~\cite{guillemot2013nonexistence} & FPT~$2.56^k$~\cite{NG12} NOSUB~\cite{drange2015exploring,DP17} & KER~$k^3$~\cite{guillemot2013nonexistence} & FPT~$2.56^k$~\cite{NG12} NOSUB~\cite{drange2015exploring,DP17} & KER~$k^3$~\cite{guillemot2013nonexistence} & FPT~$4.61^k$~\cite{LWG+12} NOSUB~\cite{DP17} \tabularnewline
\hline
\hline
split \textbf{*} & KER~$k^2$~\cite{ghosh2015faster} KER~$k^4$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{ghosh2015faster} & KER~$k^2$~\cite{ghosh2015faster} KER~$k^4$~\cite{guo2007problem} & SUB~$2^{\sqrt{k}\log k}$~\cite{ghosh2015faster} & - & - \tabularnewline
\hline
pseudosplit \textbf{*} & - & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015exploring} & - & SUB~$2^{\sqrt{k}\log k}$~\cite{drange2015exploring} & - & - \tabularnewline
\hline
proper interval & KER~$k^3$~\cite{bessy2013polynomial} & SUB~$2^{{2/3}\log k}$~\cite{bliznets2015subexponential} FPT~$4^k$~\cite{LWX15} FPT~$16^k$~\cite{kaplan1999tractability} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & - & - & - & - \tabularnewline
\hline
interval & - & SUB~$2^{\sqrt{k}\log k}$~\cite{bliznets2016subexponential} FPT~$6^k$~\cite{Cao13,cao2016linear} FPT~$4^{k\log k}$~\cite{villanger2009interval} NO~$2^{k^{1/4}}$~\cite{bliznets2016lower} & - & FPT~$2^{k\log k}$~\cite{cao2016linear} & - & - \tabularnewline
\hline
strongly chordal & - & FPT~$64^k$~\cite{kaplan1999tractability} & - & - & - & - \tabularnewline
\hline
chordal & KER~$k^3$~\cite{kaplan1999tractability} & SUB~$2^{\sqrt{k}\log k}$~\cite{fomin2013subexponential} FPT~$4^k$~\cite{cai1996fixedparameter} FPT~$16^k$~\cite{kaplan1999tractability} FPT~$2^{k\log k}$~\cite{cao2014chordal}  NO~$2^{\sqrt{k}}$~\cite{CS17} &  - & FPT~\cite{Mar10} FPT~$2^{k\log k}$~\cite{cao2014chordal} &  - & FPT~$2^{k\log k}$~\cite{cao2014chordal} \tabularnewline
\hline
\end{tabular}
%\end{center}
%\vspace*{-1em}
\medskip
\caption{Parameterized complexity of edge modification problems into classic hereditary graph classes. A star next to the name of the class marks autocomplemented classes, for which any result for one of the completion problem or deletion problem automatically gives the same result for the other problem. \label{tab:hered}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%




% %
% % Directed
% %
% \input{graph-classes-directed}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "survey"
%%% End:



==> introduction.tex <==
\section{Introduction}
\pause
%
Graph modification problems form an important subclass of discrete computational
problems, where the task is to modify a given graph using a constrained number
of modifications in order to make it satisfy some property~$\Pi$, or
equivalently belong to the class~$\mathcal{G}$ of graphs satisfying~$\Pi$.
Well-known examples of graph modification problems include \pname{Vertex Cover},
\pname{Cluster Editing}, \pname{Feedback Vertex Set}, \pname{Odd Cycle
  Transversal}, and \pname{Minimum Fill-In}.  The systematic study of graph
modification problems dates back to early 80s and the work of
Yannakakis~\cite{yannakakis1981edgedeletion}, who showed that there is a
dichotomy for the vertex deletion problems: unless a graph class~$\mathcal{G}$
is trivial (finite or co-finite), the problem of deleting the least number of
vertices to obtain a graph from~$\mathcal{G}$ is \NP-hard.
%
Mutatis mutandis for the edge case, but in order to obtain a graph
from~$\mathcal{G}$, we are to modify the edge set of the graph instead of the
vertex set, there are three natural classes of problems: deletion problems
(deleting the least number of edges), completion problems (adding the least
number of edges) and editing problems (performing the least number of edge
additions or deletions).



\bigpause
% 
The purpose of this survey is to summarize parts of the history of edge
modification, with a focus on the parameterized and kernelization complexity.
This is not the first study of graph modification problems, see for instance the
work by Burzyn, Bonomo and Dur{\'a}n~\cite{burzyn2006npcompleteness} on edge
modification problems, and the thesis \emph{Graph modification problems related
  to graph classes} by Mancini~\cite{mancini2008graph} for good overview of the
classical complexity of graph modification problems.
%
For completeness, we also mention that there was a short survey on the
kernelization complexity by Liu, Wang and Guo~\cite{liu2014overview}, but this
work was less of a historical approach, and more an investigative approach
exploring the frontier of the kernelization complexity of graph modification
problems.
%
See also the survey by Brandstädt, Le, and Spinrad on graph
classes~\cite{brandstadt1999graph}.

\medpause
%
For an introduction to parameterized complexity analysis, see monographs Downey
Fellows~\cite{downey1999parameterized, downey2013fundamentals}, Flum
Grohe~\cite{flum2006parameterized} or
Niedermeier~\cite{niedermeier2006invitation}.






\paragraph{The optimality programme.}
% 
Once a problem has been shown to admit a fixed-parameter tractable algorithm, a
natural next question is whether it is possible to improve upon that algorithm.
This is especially interesting when the algorithms have nasty running times like
$2^{O(k^2)} \cdot \poly(n)$, or even $2^{O(2^k)} \cdot \poly(n)$.
% 
As mentioned above, the modification problems for finite forbidden induced
subgraphs already have nice running times like $6^k \cdot \poly(n)$ or even $3^k
\cdot \poly(n)$.  Is it possible to obtain faster algorithms than what Cai's
theorem provides?  Can we improve from $3^k\poly(n)$ to, say, $2^k\poly(n)$ or
$1.5^k\poly(n)$?
\begin{quote}
  Clearly, it would be very useful to know if the current best algorithm can be
  improved further or it has already hit some fundamental barrier.
  % 
  \\ --- Marx~\cite{marx2012whats}.
\end{quote}

\noindent
% 
As Marx points out, it would be interesting to see if there are reasons to
suspect that we cannot get better than $2^k\cdot\poly(n)$ algorithms.
%
We will return to that question later and indeed throughout this thesis, but
first we take a detour into the world of compression and preprocessing.



==> macros.tex <==
\usepackage{accsupp}

\makeatletter
\DeclareRobustCommand{\generic}{%
  \BeginAccSupp{ActualText=Generic}\textsf{Gener\istar c}\EndAccSupp{}}
\newcommand{\istar}{%
  \leavevmode
  \vbox{%
    \offinterlineskip
    \ialign{\hfil##\hfil\cr\hidewidth$\scriptstyle\star$\hidewidth\cr\i\cr}%
  }%
}
\makeatother


\makeatletter
\DeclareRobustCommand{\Friendface}{%
  \BeginAccSupp{ActualText=Friendface}\textsf{Fr\istar endface}\EndAccSupp{}}
\makeatother

% \usepackage{stackengine}
% \def\asterism{\par\vspace{1em}{\centering\scalebox{1.5}{%
%   \stackon[-0.5pt]{\bfseries*~*}{\bfseries*}}\par}\vspace{.5em}\par}

\newcommand{\majorpause}{\bigskip\bigskip\bigskip\bigskip\noindent} % del \asterism

\newcommand{\bigpause}{\bigskip\noindent}
\newcommand{\medpause}{\medskip\noindent}
\newcommand{\smallpause}{\smallskip\noindent} \newcommand{\pause}{\bigpause}





%
% THEOREMS
%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{open}{Open problem}[section]

\theoremstyle{remark}
\newtheorem{redrule}{Rule}
\newtheorem{definition}{Definition}[section]












\DeclareMathOperator{\fn}{fn}
\DeclareMathOperator{\am}{am} % adjacency matrix
\DeclareMathOperator{\rank}{rank}

\def\cqedsymbol{\ifmmode$\lrcorner$\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil$\lrcorner$
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi} 

\newcommand{\cqed}{\renewcommand{\qed}{\cqedsymbol}}

\newcommand{\gpath}[1]{{\langle #1 \rangle}}          % graph path: used for paths
%\newcommand{\gcycle}[1]{{\langle #1 \rangle_{\circ}}} % graph cycle: used for cycles
\newcommand{\gcycle}{\gpath}

\newcommand{\pname}{\textsc}
\newcommand{\gclass}[1]{\textnormal{\textbf{#1}}}
\newcommand{\cclass}[1]{\textsf{\textup{#1}}}


\newcommand{\NP}{\cclass{NP}\xspace}
\newcommand{\np}{\NP\xspace}
\newcommand{\NPc}{\cclass{NPc}\xspace}

\newcommand{\XP}{\cclass{XP}\xspace}

\newcommand{\pt}{\cclass{P}} % for the tables

\newcommand{\npci}{\cclass{NP}-complete\xspace}
\newcommand{\paraNP}{\cclass{Para-NP}\xspace}

\newcommand{\FPT}{\cclass{FPT}\xspace}
\newcommand{\fpt}{\FPT}

\newcommand{\SUBEPT}{\cclass{SUBEPT}\xspace}

\newcommand{\WOne}{\cclass{W[1]}\xspace}
\newcommand{\wone}{\WOne\xspace}

\newcommand{\WTwo}{\cclass{W[2]}\xspace}
\newcommand{\wtwo}{\WTwo\xspace}

\newcommand{\yesinstance}{yes-instance\xspace}
\newcommand{\noinstance}{no-instance\xspace}
\newcommand{\ETH}{ETH\index{exponential time hypothesis}}
\newcommand{\polyn}{n^{\Oh(1)}}

%%% Big-O 
\newcommand{\Ostar}{O^\star}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\Oh}{\cO}
\newcommand{\cOs}{\mathcal{O}^*}
\newcommand{\Ohstar}{\cOs}




% poly hierarchy collapse
\newcommand{\PNP}{$\cclass{P} = \cclass{NP}$}%
\newcommand{\pnp}{\PNP}

% poly hierarchy collapse
\newcommand{\PH}{$\cclass{NP} \subseteq \cclass{coNP/poly}$%
\index{PHcoNP/poly@$\cclass{NP} \subseteq \cclass{coNP/poly}$}}

\newcommand{\ph}{\PH}

\newcommand{\NOPH}{$\cclass{NP} \not\subseteq \cclass{coNP/poly}$%
\index{PHxcoNP/poly@$\cclass{NP} \not\subseteq \cclass{coNP/poly}$}}

\newcommand{\noph}{\NOPH}

\newcommand{\corp}{co-\cclass{RP}} % co-RP kernel


\newcommand{\KW}{\ensuremath{H_{\text{KW}}}} % The KW graph, Kratsch and Wahlström

\newcommand{\funfamily}{\mathfrak{F}}

\newcommand{\symdiff}{\vartriangle}%\triangle
\newcommand{\edges}[1][V]{\left[#1\right]^2} % use: \edges=\edges[V] or \edges[V']


\newcommand{\G}{\mathcal{G}}
\newcommand{\C}{\mathcal{C}}

\newcommand{\I}{\mathcal{I}}
\newcommand{\V}{\mathcal{V}}

\newcommand{\TP}{\mathcal{TP}}
%\renewcommand{\H}{\mathcal{H}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\sm}{\setminus}
\newcommand{\bigO}{O}
% \newcommand{\Ostar}{\mathcal{O}^\star}
% \newcommand{\Otilde}{\tilde{{\O}}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\phi}{\varphi}

\newcommand{\osl}{\ensuremath{{O(\sqrt{k} \log{k})}}}


%
% PROBLEM NAMES
%
\newcommand{\SAT}{\pname{3Sat}}

\newcommand{\TrivPC}{\pname{Trivially Perfect Completion}}
\newcommand{\TrivPD}{\pname{Trivially Perfect Deletion}}
\newcommand{\TrivPE}{\pname{Trivially Perfect Editing}}


\newcommand{\CoC}{\pname{Cograph Completion}}
\newcommand{\CoD}{\pname{Cograph Deletion}}
\newcommand{\CoE}{\pname{Cograph Editing}}

\newcommand{\CFourC}{\pname{$C_4$-free Completion}}
\newcommand{\CFourD}{\pname{$C_4$-free Deletion}}
\newcommand{\CFourE}{\pname{$C_4$-free Editing}}



\newcommand{\BicE}{\pname{Bicluster Editing}}
\newcommand{\StarE}{\pname{Starforest Editing}}

\newcommand{\PStarE}{\pname{$p$-Starforest Editing}\index{p-Starforest Editing@\pname{$p$-Starforest Editing}}}
\newcommand{\PBicE}{\pname{$p$-Bicluster Editing}\index{p-Bicluster Editing@\pname{$p$-Bicluster Editing}}}
\newcommand{\TpartBE}{\pname{$t$-partite $p$-cluster Editing}\index{t-partite
    p-cluster editing@\pname{$t$-partite $p$-cluster Editing}}} % % t-partite p-cluster editing


\newcommand{\SplitC}{\pname{Split Completion}}
\newcommand{\SplitD}{\pname{Split Deletion}}
\newcommand{\SplitE}{\pname{Split Editing}}


\newcommand{\ThreshC}{\pname{Threshold Completion}}
\newcommand{\ThreshD}{\pname{Threshold Deletion}}
\newcommand{\ThreshE}{\pname{Threshold Editing}}

\newcommand{\SplitTE}{\pname{Split Threshold Editing}}

\newcommand{\ChainC}{\pname{Chain Completion}}
\newcommand{\ChainD}{\pname{Chain Deletion}}
\newcommand{\ChainE}{\pname{Chain Editing}}

\newcommand{\ChordC}{\probChordComp}
\newcommand{\ChordD}{\pname{Chordal Deletion}}
\newcommand{\ChordE}{\pname{Chordal Editing}}

\newcommand{\CobiChordE}{\pname{Cobipartite Chordal Editing}}

\newcommand{\BipChainE}{\pname{Bipartite Chain Editing}}

\newcommand{\PseudoC}{\pname{Pseudosplit Completion}}
\newcommand{\PseudoD}{\pname{Pseudosplit Deletion}}
\newcommand{\PseudoE}{\pname{Pseudosplit Editing}}









\DeclareMathOperator{\diam}{diam} % diameter
\DeclareMathOperator{\dist}{dist}

\DeclareMathOperator{\poly}{poly} % poly(k)
\DeclareMathOperator{\polylog}{polylog} % poly(k)

\DeclareMathOperator{\dpt}{dp}    % DP table
\DeclareMathOperator{\en}{en}    % editing number






%
%
%  def (par) problem
%
%
%%%%% BEGIN FELIX %%%%%%%%%%%%

\newlength{\RoundedBoxWidth}
\newsavebox{\GrayRoundedBox}
\newenvironment{GrayBox}[1]%
   {\setlength{\RoundedBoxWidth}{.93\textwidth}
    \def\boxheading{#1}
    \begin{lrbox}{\GrayRoundedBox}
       \begin{minipage}{\RoundedBoxWidth}}%
   {   \end{minipage}
    \end{lrbox}
    \begin{center}
    \begin{tikzpicture}%
       \node(Text)[draw=black!20,fill=white,rounded corners,%
             inner sep=2ex,text width=\RoundedBoxWidth]%
             {\usebox{\GrayRoundedBox}};
        \coordinate(x) at (current bounding box.north west);
        \node [draw=white,rectangle,inner sep=3pt,anchor=north west,fill=white] 
        at ($(x)+(6pt,.75em)$) {\boxheading};
    \end{tikzpicture}
    \end{center}}     

\newenvironment{defproblemx}[2][]{\noindent\ignorespaces%
                                \FrameSep=6pt%
                                \parindent=0pt%
                \vspace*{-1.5em}
                \ifthenelse{\isempty{#1}}{%
                  \begin{GrayBox}{\textsc{#2}}%                
                }{%
                   \begin{GrayBox}{\textsc{#2} %parameterized by~{#1}
                   }%  
                }
                \newcommand\Prob{Problem:}%
                \newcommand\Input{Input:}%                        
                \begin{tabular*}{\textwidth}{@{\hspace{.1em}} >{\itshape} p{1.8cm} p{0.8\textwidth} @{}}%        
            }{
                \end{tabular*}%
                \end{GrayBox}%
                \ignorespacesafterend
            }  

\newcommand{\defparproblem}[4]{% FJR Version
  \begin{defproblemx}[#2]{#1}
    Input:  & #3 \\
    Task: & #4
  \end{defproblemx}
}%

\newcommand{\defproblem}[3]{% FJR Version
  \begin{defproblemx}{#1}
    Input:  & #2 \\
    Question: & #3
  \end{defproblemx}
}%

%%%%% END FELIX %%%%%%%%%%%%










\newcommand{\wei}{\mathbf{w}}


\DeclareMathOperator{\uni}{uni}
\DeclareMathOperator{\mc}{mc}


\newcommand{\subindeq}{\trianglelefteq}
\newcommand{\iso}{\cong}
\newcommand{\app}{$\spadesuit$} % \star ?


\DeclareMathOperator{\tw}{tw}
\DeclareMathOperator{\pw}{pw}
\DeclareMathOperator{\td}{td}
\DeclareMathOperator{\vc}{vc}
\newcommand{\vpmc}{vital potential maximal clique}
\newcommand{\Vpmc}{Vital potential maximal clique\index{vital potential maximal clique}}


\newcommand{\third}{\gemini}  % These two are used in the tp reduction %
\newcommand{\paw}{\mathsf{P}} % These two are used in the tp reduction

\newcommand{\tpss}{weakly laminar set system\index{weakly laminar set system}}
\newcommand{\Tpss}{Weakly laminar set system\index{weakly laminar set system}}


\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\del}{\partial}

\DeclareMathOperator{\cost}{cost} % DP table










%
% FOR THE TABLE
%


\newcommand{\miss}{$\times$}
\newcommand{\openq}{open}
\newcommand{\csq}{\ensuremath{c^{\sqrt k \log k}}}


\newcommand{\entry}[4]{\begin{tabular}[c]{@{}l@{}}{#1}\\ {#2} \textbar{} {#3}\\ {#4}\end{tabular}}
\newcommand{\pentry}[1][]{\begin{tabular}[c]{@{}l@{}}{\cclass{P}~{#1}}\\ \mbox{} \\ \mbox{} \end{tabular}}

% Generic 3 line entry
\newcommand{\trientry}[3]{\begin{tabular}[c]{@{}l@{}}{{#1}}\\ {#2} \\ {#3}\end{tabular}}


% \npentry{2^k}{No}{k^3}
\newcommand{\npentry}[4]{\entry{\NPc~#1}{#2}{#3}{#4}}
\newcommand{\npentryyanna}[3]{\entry{\NPc~\cite{yannakakis1978node}}{#1}{#2}{#3}}


% \nosubentry{np-cite}{2^k}{no-cite}{k^3}
\newcommand{\nosubentry}[4]{\npentry{#1}{#2}{No~#3}{#4}}


% \subentry{np-cite}{\csq}{k^3}
\newcommand{\subentry}[3]{\trientry{\NPc~{#1}}{#2}{#3}}

















% OLD
% OLD
% OLD
% OLD
% OLD


\newcommand{\F}{\ensuremath{\mathcal{F}}}

% \newcommand{\pname}{\textsc}
% \newcommand{\cclass}[1]{\textsf{\textup{#1}}}
% \newcommand{\NP}{\cclass{NP}}
% \newcommand{\np}{\NP}
% \newcommand{\NPc}{\cclass{NPc}}
% \newcommand{\npc}{\NPc}

% \newcommand{\WOne}{\cclass{W[1]}}
% \newcommand{\wone}{\WOne}
% \newcommand{\wtwo}{\cclass{W[2]}}

% \newcommand{\Ostar}{O^\star}
% \newcommand{\ostar}{\Ostar}


% poly hierarchy collapse
% \newcommand{\PH}{$\cclass{NP} \subseteq \cclass{coNP/poly}$}
% \newcommand{\ph}{\PH}

% \newcommand{\NOPH}{$\cclass{NP} \not\subseteq \cclass{coNP/poly}$}
% \newcommand{\noph}{\NOPH}


%%%%%%%%%%%
%%problem names
\newcommand{\ProblemFormat}[1]{\pname{#1}}
\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}{}\xspace}

 %\newcommand{\ProblemFormat}[1]{{\sc #1}}

%\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
%\newcommand{\ProblemIndexBeg}[1]{\index{problem!\ProblemFormat{#1}|(}}
%\newcommand{\ProblemIndexEnd}[1]{\index{problem!\ProblemFormat{#1}|)}}

%\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}\xspace}
%\newcommand{\ProblemNameX}[2]{\ProblemFormat{#1}\ProblemIndex{#2}\xspace}




 

%\newcommand{\probDCluster}{\ProblemName{$d$-Clustering}}
%\newcommand{\probCedit}{\ProblemName{Cluster Editing}}

\newcommand{\BE}{\pname{Bicluster Editing}}
\newcommand{\be}{\BE}

\newcommand{\pbe}{\pname{$p$-Bicluster Editing}}
\newcommand{\tpe}{\pname{$t$-Partite $p$-Cluster Editing}}
\newcommand{\te}{\pname{$t$-Partite Cluster Editing}}

\newcommand{\SE}{\pname{Starforest Editing}}
\newcommand{\se}{\SE}

\newcommand{\pse}{\pname{$p$-Starforest Editing}}


\newcommand{\HVD}{\pname{$\mathcal{H}$-Free Vertex Deletion}}

\newcommand{\HED}{\pname{$\mathcal{H}$-Free Deletion}}
\newcommand{\HEE}{\pname{$\mathcal{H}$-Free Editing}}
\newcommand{\HEC}{\pname{$\mathcal{H}$-Free Completion}}
\newcommand{\hed}{\HED}
\newcommand{\hee}{\HEE}
\newcommand{\hec}{\HEC}




\renewcommand{\phi}{\varphi}





%\newcommand{\edges}[1][V]{\binom{#1}{2}} % use: \edges=\edges[V] or \edges[V']
%\newcommand{\edges}[1][V]{\left[#1\right]^2} % use: \edges=\edges[V] or \edges[V']

%%%%%%%%%%%%%%%%%%%
%% Problem names
%%%%%%%%%%%%%%%%%%%
 

% Commonly used names
\newcommand{\probVC}{\ProblemName{Vertex Cover}}
\newcommand{\probPlVC}{\ProblemName{Planar Vertex Cover}}
\newcommand{\probPVC}{\ProblemName{Partial Vertex Cover}}
\newcommand{\probPDS}{\ProblemName{Partial Dominating Set}}
\newcommand{\probFVS}{\ProblemName{Feedback Vertex Set}}
\newcommand{\probIFVS}{\ProblemName{Independent Feedback Vertex Set}}
\newcommand{\probCycPacking}{\ProblemName{Cycle Packing}}
\newcommand{\probPlFVS}{\ProblemName{Planar Feedback Vertex Set}}
\newcommand{\probIS}{\ProblemName{Independent Set}}
\newcommand{\probWIS}{\ProblemName{Weighted Independent Set}}
\newcommand{\probMCIS}{\ProblemName{Multicolored Independent Set}}
\newcommand{\probDS}{\ProblemName{Dominating Set}}
%\newcommand{\probMDS}{\ProblemName{Minimum Dominating Set}}
\newcommand{\probPlDS}{\ProblemName{Planar Dominating Set}}
\newcommand{\probCDS}{\ProblemName{Connected Dominating Set}}
\newcommand{\probDST}{\ProblemName{Dominating Set on Tournaments}}
\newcommand{\probClique}{\ProblemName{Clique}}
\newcommand{\probMC}{\ProblemName{Multicolored Clique}}
\newcommand{\probPClique}{\ProblemName{Partitioned Clique}}
\newcommand{\probqSC}{\ProblemName{$q$-Set Cover}}
\newcommand{\probSC}{\ProblemName{Set Cover}}
\newcommand{\probDSP}{\ProblemName{Dominating Set with Pattern}}
\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probHam}{\ProblemName{Hamiltonian Cycle}}
\newcommand{\probPlHam}{\ProblemName{Planar Hamiltonian Cycle}}
\newcommand{\probHamP}{\ProblemName{Hamiltonian Path}}
\newcommand{\probKPath}{\ProblemName{Longest Path}}
\newcommand{\probWKPath}{\ProblemName{Weighted Longest Path}}
\newcommand{\probthreeSAT}{\ProblemName{$3$-SAT}}
\newcommand{\probqSAT}{\ProblemName{$q$-SAT}}
\newcommand{\probcnfSAT}{\ProblemName{CNF-SAT}}
\newcommand{\probthreeCol}{\ProblemName{$3$-Coloring}}
\newcommand{\probqCol}{\ProblemName{$q$-Coloring}}
\newcommand{\probListColoring}{\ProblemName{List Coloring}}
\newcommand{\probOddSet}{\ProblemName{Odd Set}}
\newcommand{\probTuring}{\ProblemName{Short Turing Machine Acceptance}}
\newcommand{\probSI}{\ProblemName{Subgraph Isomorphism}}
\newcommand{\probGI}{\ProblemName{Graph Isomorphism}}
\newcommand{\probWCS}{\ProblemName{Weighted Circuit Satisfiability}}
\newcommand{\probClosestString}{\ProblemName{Closest String}}
\newcommand{\probClosestSubstring}{\ProblemName{Closest Substring}}
\newcommand{\probGridTiling}{\ProblemName{Grid Tiling}}
\newcommand{\probGridTilingLeq}{\ProblemName{Grid Tiling with~$\le$}}
\newcommand{\probUnitDisk}{\ProblemName{Unit Disk Independent Set}}
\newcommand{\probEMWay}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probEDS}{\ProblemName{Edge Dominating Set}}
\newcommand{\probEMWaySets}{\ProblemName{Edge Multiway Cut for Sets}}
\newcommand{\probDirEMWay}{\ProblemName{Directed Edge Multiway Cut}}
\newcommand{\probEMCut}{\ProblemName{Edge Multicut}}
\newcommand{\probMulticut}{\ProblemName{Multicut}}
\newcommand{\probDirEMCut}{\ProblemName{Directed Edge Multicut}}
\newcommand{\probSkewEMCut}{\ProblemName{Skew Edge Multicut}}
\newcommand{\probDFVS}{\ProblemName{Directed Feedback Vertex Set}}
\newcommand{\probDFAS}{\ProblemName{Directed Feedback Arc Set}}
\newcommand{\probDFASC}{\ProblemName{Directed Feedback Arc Set Compression}}
\newcommand{\probPartpq}{\ProblemName{$(p,q)$-Partition}}
\newcommand{\probClusterpq}{\ProblemName{$(p,q)$-Cluster}}
\newcommand{\probSatellite}{\ProblemName{Satellite Problem}}
\newcommand{\probTw}{\ProblemName{Treewidth}}
\newcommand{\probPerfSetMatch}{\ProblemName{Perfect $d$-Set Matching}}
\newcommand{\probHS}{\ProblemName{Hitting Set}}
\newcommand{\probdHS}{\ProblemName{$d$-Hitting Set}}
\newcommand{\probEdHS}{\ProblemName{E$d$-Hitting Set}}
\newcommand{\probSetSplit}{\ProblemName{Set Splitting}}
\newcommand{\probSteiner}{\ProblemName{Steiner Tree}}
\newcommand{\probSteinerF}{\ProblemName{Steiner Forest}}
\newcommand{\probMotif}{\ProblemName{Graph Motif}}
\newcommand{\probColorfulMotif}{\ProblemName{Colorful Graph Motif}}
\newcommand{\probRBDSlong}{\ProblemName{Red-Blue Dominating Set}}
\newcommand{\probRBDS}{\ProblemNameX{RBDS}{Red-Blue Dominating Set}}
\newcommand{\probCRBDSlong}{\ProblemName{Colored Red-Blue Dominating Set}}
\newcommand{\probCRBDS}{\ProblemNameX{Col-RBDS}{Colored Red-Blue Dominating Set}}
\newcommand{\probCVC}{\ProblemName{Connected Vertex Cover}}
\newcommand{\probCFVS}{\ProblemName{Connected Feedback Vertex Set}}
\newcommand{\probCBullHit}{\ProblemName{Connected Bull Hitting}}
\newcommand{\probSetPacking}{\ProblemName{Set Packing}}
\newcommand{\probDisFactors}{\ProblemName{Disjoint Factors}}
\newcommand{\probDisPaths}{\ProblemName{Vertex Disjoint Paths}}
\newcommand{\probChromatic}{\ProblemName{Chromatic Number}}
\newcommand{\probECC}{\ProblemName{Edge Clique Cover}}
\newcommand{\probSubsetSum}{\ProblemName{Subset Sum}}
\newcommand{\probKnapsack}{\ProblemName{Knapsack}}
\newcommand{\probWayCut}{\ProblemName{$s$-Way Cut}}
\newcommand{\probEulerian}{\ProblemName{Eulerian  Deletion}}
\newcommand{\probBisec}{\ProblemName{Minimum Bisection}}
\newcommand{\probMaxBisec}{\ProblemName{Maximum Bisection}}

\newcommand{\probHalt}{\ProblemName{Halting}}

\newcommand{\probbarF}{\ProblemName{Bar Fight Prevention}}

\newcommand{\probCountMatchings}{\ProblemName{\#Perfect Matchings}}
\newcommand{\probCountSteiner}{\ProblemName{\#Steiner Tree}}
\newcommand{\probCountHam}{\ProblemName{\#Hamiltonian Cycle}}


\newcommand{\probMaxLeafSubtree}{\ProblemName{Max Leaf Subtree}}
\newcommand{\probMaxSat}{\ProblemName{Maximum Satisfiability}}
\newcommand{\probMaxrSat}{\ProblemName{Max-$r$-SAT}}
\newcommand{\probMaxErSat}{\ProblemName{Max-E$r$-SAT}}

\newcommand{\probIndMat}{\ProblemName{Induced Matching}}
\newcommand{\probMaxFlow}{\ProblemName{Maximum Flow}}

\newcommand{\probVertexColoring}{\ProblemName{Vertex Coloring}}
%%% Section 1

\newcommand{\mctodo}[1]{\todo[inline, linecolor=green!70!white, backgroundcolor=blue!20!white, bordercolor=red]{MC: #1}}
\newcommand{\dmtodo}[1]{\todo[inline, linecolor=green!70!white, backgroundcolor=blue!20!white, bordercolor=red]{DM: #1}}
\newcommand{\fftodo}[1]{\todo[inline, linecolor=green!70!white, backgroundcolor=blue!20!white, bordercolor=red]{FVF: #1}}
\newcommand{\fftodoA}[1]{\todo[linecolor=green!70!white, backgroundcolor=blue!20!white, bordercolor=red]{FVF: #1}}
\newcommand{\probFASTfull}{\ProblemName{Feedback Arc Set in Tournaments}}
\newcommand{\probFAST}{\ProblemNameX{FAST}{Feedback Arc Set in Tournaments}}
\newcommand{\probCochromatic}{\ProblemName{Cochromatic Number}}
\newcommand{\probVCLP}{\ProblemName{Vertex Cover Above LP}}
\newcommand{\probPi}{\ProblemName{$\mathrm{\Pi}$-Vertex Deletion}}
\newcommand{\probATSAT}{\ProblemName{Almost $2$-SAT}}
\newcommand{\probATSATvd}{\ProblemName{Variable Deletion Almost $2$-SAT}}
\newcommand{\probDFVST}{\ProblemName{Feedback Vertex Set in Tournaments}}
\newcommand{\probDFVSTshort}{\ProblemNameX{FVST}{Feedback Vertex Set in Tournaments}}
\newcommand{\probStarCompr}{\ProblemName{($*$)-Compression}}
\newcommand{\probStarDisj}{\ProblemName{Disjoint-($*$)}}
\newcommand{\probDisjVC}{\ProblemName{Disjoint Vertex Cover}}
\newcommand{\probDFVSTCompr}{\ProblemName{Feedback Vertex Set in Tournaments Compression}}
\newcommand{\probDFVSTDisj}{\ProblemName{Disjoint Feedback Vertex Set in Tournaments}}
\newcommand{\probKTree}{\ProblemName{$k$-Tree}}
\newcommand{\probDCluster}{\ProblemName{$d$-Clustering}}
\newcommand{\probTSP}{\ProblemName{TSP}}
\newcommand{\probMaxCut}{\ProblemName{MaxCut}}


\newcommand{\probCVD}{\ProblemName{Cluster Vertex Deletion}}
\newcommand{\probCedit}{\ProblemName{Cluster Editing}}
\newcommand{\probChordComp}{\ProblemName{Chordal Completion}}
\newcommand{\probMMM}{\ProblemName{Minimum Maximal Matching}}
\newcommand{\probdBDD}{\ProblemName{$d$-Bounded-Degree Deletion}}
\newcommand{\probDualCol}{\ProblemName{Dual-Coloring}}
\newcommand{\probSVD}{\ProblemName{Split Vertex Deletion}}
\newcommand{\probEDCP}{\ProblemName{Edge Disjoint Cycle Packing}}
\newcommand{\probMIST}{\ProblemName{Max-Internal Spanning Tree}}
\newcommand{\probRamsey}{\ProblemName{Ramsey}}
\newcommand{\probMinonerSat}{\ProblemName{Min-Ones-$r$-SAT}}
\newcommand{\probMinonetwoSat}{\ProblemName{Min-Ones-$2$-SAT}}
\newcommand{\probMintwoSat}{\ProblemName{Min-$2$-SAT}}
\newcommand{\probMaxLeafSptree}{\ProblemName{Max Leaf Spanning Tree}}
\newcommand{\probDMaxLeaf}{\ProblemName{Directed Max Leaf}}
\newcommand{\probVCparamOCT}{\ProblemName{Vertex Cover/OCT}}
\newcommand{\probMinCut}{\ProblemName{Min-Cut}}

\newcommand{\probPLC}{\ProblemName{Point Line Cover}}

 
\newcommand{\allHalf}{all-$\frac{1}{2}$-solution}

%\newcommand{\vc}{\operatorname{vc}}
 
\newcommand{\LPVC}{LPVC}

\newcommand{\probtwoSAT}{\ProblemName{$2$-SAT}}
\newcommand{\probVCaboveMatch}{\ProblemName{Vertex Cover Above Matching}}
\newcommand{\probDisjFVS}{\ProblemName{Disjoint Feedback Vertex Set}}
\newcommand{\probDisjOCT}{\ProblemName{Disjoint Odd Cycle Transversal}}
\newcommand{\probAnBC}{\ProblemName{Annotated Bipartite Coloring}}
\newcommand{\probAnATSAT}{\ProblemName{Annotated Satisfiable Almost 2-SAT}}
\newcommand{\probImbalance}{\ProblemName{Imbalance}}
\newcommand{\probILP}{\ProblemName{Integer Linear Programming Feasibility}}
%\newcommand{\probILPopt}{\ProblemName{Integer Linear Programming Optimization}}
\newcommand{\probILPopt}{\ProblemName{Integer Linear Programming}}
\newcommand{\probLPopt}{\ProblemName{Linear Programming}}
\newcommand{\oct}{odd cycle transversal}

\newcommand{\probTrianglePacking}{\ProblemName{Triangle Packing}}
\newcommand{\probTreeSI}{\ProblemName{Tree Subgraph Isomorphism}}
\newcommand{\probPseudoAChr}{\ProblemName{Pseudo Achromatic Number}}
\newcommand{\probSplitED}{\ProblemName{Split Edge Deletion}}

%\newcommand{\probGenus}{\ProblemName{Euler Genus}}
\newcommand{\probGenus}{\ProblemName{Graph Genus}}
\newcommand{\probLinkless}{\ProblemName{Linkless Embedding}}
\newcommand{\probPlanDiam}{\ProblemName{Planar Diameter Improvement}}
\newcommand{\probFaceCover}{\ProblemName{Face Cover}}


\newcommand{\fvs}{feedback vertex set}
\newcommand{\dfvs}{directed feedback vertex set}
\newcommand{\probthreeHS}{\ProblemName{$3$-Hitting Set}}

\DeclareMathOperator{\operatorPATH}{PATH}


% Derandomization, splitters etc.
\newcommand{\splitter}{\mathcal{F}}
\newcommand{\splitfun}{f}
\newcommand{\splitK}{k}
\newcommand{\splitL}{\ell}
\newcommand{\univset}{\mathcal{U}}

% Set cover, Steiner tree
\newcommand{\scU}{U}
\newcommand{\scF}{\mathcal{F}}
\newcommand{\stTerms}{K}
\newcommand{\stTree}{H}

% Any surface
\newcommand{\surface}{\Sigma}
% Minor relation
\newcommand{\leqM}{\leq_m}
% forbidden graphs
\DeclareMathOperator{\operatorForb}{Forb}
\newcommand{\forb}{\ensuremath{\operatorForb}}

\newcommand{\pluskv}[1]{\ensuremath{#1+k\mathrm{v}}}
\newcommand{\probGvd}{\ProblemName{$\GG$ Vertex Deletion}}
\newcommand{\probGkvRecog}{\ProblemName{$\pluskv{\GG}$ Recognition}}
 

%%%%Intro
\newcommand{\probPedel}{\ProblemName{$\mathcal{G}$-Edge  Deletion}}
\newcommand{\probPedad}{\ProblemName{$\mathcal{G}$-Edge  Completion}}
\newcommand{\probPeded}{\ProblemName{$\mathcal{G}$-Edge  Editing}}


%%% Section 2
%%%%%%%
\newcommand{\MSO}{\ensuremath{\mathbf{MSO}}}
\newcommand{\FO}{\ensuremath{\mathbf{FO}}}
\newcommand{\probrCentert}{\ProblemName{$r$-Center}}
\newcommand{\probPlanDel}{\ProblemName{Planar Vertex Deletion}}
\newcommand{\probPlanDelCompr}{\ProblemName{Planar Deletion Compression}}
\newcommand{\probTreeSpan}{\ProblemName{Tree Spanner}}
\newcommand{\probKCycle}{\ProblemName{Longest Cycle}}
\newcommand{\probPlKPath}{\ProblemName{Planar Longest Path}}
%\newcommand{\probPlDS{\ProblemName{Planar Dominating Set}}
\newcommand{\probPlKCycle}{\ProblemName{Planar Longest Cycle}}
\newcommand{\probTWdel}{\ProblemName{Treewidth-$\eta$ Modulator}}
\newcommand{\probBidMin}{\ProblemName{$\phi$-Minimization}}
\newcommand{\probBidMax}{\ProblemName{$\phi$-Maximization}}
\newcommand{\probAnnPlanDelCompr}{\ProblemName{Disjoint Planar Vertex Deletion}}

%%% Section 3
\newcommand{\probVMWay}{\ProblemName{Vertex Multiway Cut}}
\newcommand{\probVMCut}{\ProblemName{Vertex Multicut}}
\newcommand{\probDirVMWay}{\ProblemName{Directed Vertex Multiway Cut}}
\newcommand{\probDiPairCut}{\ProblemName{Digraph Pair Cut}}

%%% Section 4

\newcommand{\probPIT}{\ProblemName{Polynomial Identity Testing}}

%%% Section 5

\newcommand{\probTDS}{\ProblemName{Total Dominating Set}}

%%% Section 6

\DeclareMathOperator{\operatorOdd}{odd}
\DeclareMathOperator{\operatorDf}{df}


%%% Section 7

\newcommand{\probdMatEdSetPacking}{\ProblemName{Matroid E$d$-Set Packing}}

\newcommand{\probEllMatroidIntersection}{\ProblemName{$\ell$-Matroid Intersection}}
\newcommand{\probTwoMatroidIntersection}{\ProblemName{$2$-Matroid Intersection}}
\newcommand{\probThreeMatroidIntersection}{\ProblemName{$3$-Matroid Intersection}}
\newcommand{\probMatroidParity}{\ProblemName{Matroid Parity}}

\newcommand{\probSpecDisFVS}{\ProblemName{Special Disjoint FVS}}

\newcommand{\probdSetPacking}{\ProblemName{$d$-Set Packing}}
\newcommand{\probEdSetPacking}{\ProblemName{E$d$-Set Packing}}

\newcommand{\probLongDirCycle}{\ProblemName{Long Directed Cycle}}
\newcommand{\probLongDirPath}{\ProblemName{Longest Path}}

\newcommand{\probMaxMatching}{\ProblemName{Maximum Matching}}
\newcommand{\probBipartiteMatching}{\ProblemName{Bipartite Matching}}

%%% Section 8


 \newcommand{\probCliqueLog}{\ProblemName{$\textup{\sc Clique}_{\log}$}}
 \newcommand{\probBalancedVertexSeparator}{\ProblemName{Balanced
     Vertex Separator}}
\newcommand{\probScatteredSet}{\ProblemName{Scattered Set}}
\newcommand{\probIM}{\ProblemName{Induced Matching}}
\newcommand{\probIDS}{\ProblemName{Independent Dominating Set}}

\newcommand{\probUHS}{\ProblemName{Unique Hitting Set}}
\newcommand{\probEUHS}{\ProblemName{Exact Unique Hitting Set}}
\newcommand{\probEOddSet}{\ProblemName{Exact Odd Set}}
\newcommand{\probEEvenSet}{\ProblemName{Exact Even Set}}
\newcommand{\probEvenSet}{\ProblemName{Even Set}}
\newcommand{\probPerfectCode}{\ProblemName{Perfect Code}}

\newcommand{\probDirSteiner}{\ProblemName{Directed Steiner Tree}}
\newcommand{\probSCSS}{\ProblemName{Strongly Connected Steiner Subgraph}}

\newcommand{\probHall}{\ProblemName{Hall Set}}
\newcommand{\probVkway}{\ProblemName{Vertex $k$-Way Cut}}
\newcommand{\probTwodegVD}{\ProblemName{$2$-degenerate Vertex Deletion}}

\newcommand{\probExactCnfSat}{\ProblemName{Exact CNF-SAT}}
\newcommand{\probPerms}{\ProblemName{Permutation Composition}}
\newcommand{\probLCS}{\ProblemName{Longest Common Subsequence}}
\newcommand{\probLongIndPath}{\ProblemName{Long Induced Path}}
\newcommand{\probMBC}{\ProblemName{Multicolored Biclique}}
\newcommand{\probBiclique}{\ProblemName{Biclique}}

%%% Section 9

\newcommand{\naeSAT}{\ProblemName{NAE-SAT}}
\newcommand{\tsat}{\probthreeSAT}
\newcommand{\qsat}{\probqSAT}
\newcommand{\cnfsat}{\probcnfSAT}
\newcommand{\probPlthreeSAT}{\ProblemName{Planar $3$-SAT}}
\newcommand{\probPlthreeCol}{\ProblemName{Planar $3$-Coloring}}
\newcommand{\probkkClique}{\ProblemName{$k\times k$ Clique}}
\newcommand{\probkkPerClique}{\ProblemName{$k\times k$ Permutation Clique}}
\newcommand{\probkkPerIS}{\ProblemName{$k\times k$ Permutation Independent Set}}
\newcommand{\probkkbrClique}{\ProblemFormat{$k\times k$ (Permutation) Clique}\ProblemIndex{$k\times k$ Clique}\ProblemIndex{$k\times k$ Permutation Clique}\xspace}
\newcommand{\probkkHS}{\ProblemName{$k\times k$ Hitting Set}}
\newcommand{\probkkPerHS}{\ProblemName{$k\times k$ Permutation Hitting Set}}
\newcommand{\probkkbrHS}{\ProblemFormat{$k\times k$ (Permutation) Hitting Set}\ProblemIndex{$k\times k$ Hitting Set}\ProblemIndex{$k\times k$ Permutation Hitting Set}\xspace}
\newcommand{\probkkHSts}{\ProblemName{$k\times k$ Hitting Set with thin sets}}
\newcommand{\probkkPerHSts}{\ProblemName{$k\times k$ Permutation Hitting Set with thin sets}}
\newcommand{\probkkPerHStsdouble}{\ProblemNameX{$2k\times 2k$ Permutation Hitting Set with thin sets}{$k\times k$ Permutation Hitting Set with thin sets}}
\newcommand{\probkkbrHSts}{\ProblemFormat{$k\times k$ (Permutation) Hitting Set with thin sets}\ProblemIndex{$k\times k$ Hitting Set with thin sets}\ProblemIndex{$k\times k$ Permutation Hitting Set with thin sets}\xspace}
\newcommand{\probkkbperIS}{\ProblemName{$2k\times 2k$ Bipartite Permutation Independent Set}}
\newcommand{\probDistortion}{\ProblemName{Distortion}}
\newcommand{\probCompIntegrity}{\ProblemName{Component Order Integrity}}
%%% Section 10
\newcommand{\probMaxCycleCover}{\ProblemName{Maximum Cycle Cover}}

\newcommand{\probUnitSquare}{\ProblemName{Unit Square Independent Set}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CHRISTOPHE'S COMMANDS %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\commentaire[1]{}
\newcommand\set[1]{\ensuremath{\{ #1 \} }}
%\renewcommand\int[1]{\ensuremath{\llbracket#1\rrbracket}}
\newcommand\curs[1]{\ensuremath{{\cal{#1}}}}

% /OLD
% /OLD
% /OLD
% /OLD
% /OLD









%%% Local Variables:
%%% mode: latex
%%% TeX-master: "survey"
%%% End:


==> notes.tex <==
\subsection{History, or: A survey}
\label{sec:kernel-history-survey}

\subsection{Infinite forbidden sets}
\label{sec:survey-infinite}


\paragraph{Permutation graphs.}
Nothing is known, except for the \NP-hardness here. \fxnote{TODO check}



\paragraph{Chordal graphs.}
\pnamei{Chordal Completion} is known to admit an $O(k^2)$ vertex
kernel~\cite{natanzon2000polynomial}, whereas for the deletion and editing
cases, things are much harder.  One reason might be that for cycles of length
$\ell$ it is necessary to have a budget of size at least $\ell - 3$ to fill,
hence the number of, and length of, cycles are bounded by the budget.  This is
not the case when we allow to delete edges, as one single deletion can delete
arbitrarily many arbitrarily long cycles.


\pnamei{Chordal Editing} has been recently shown to be \FPT, where the parameter
is the number of three types of operations, i.e., vertex deletions, edge
deletions, and edge completions~\cite{cao2014chordal}.  Again, the question
remains whether this problem admits a polynomial kernel.


Observe that for the completion problem, \pname{Chordal Editing} can in fact be
characterized in form of a finite set of forbidden subgraphs, in that if the
input graph has a large enough cycle (length $k+4$), the input is a no instance.



\paragraph{Interval graphs.}
For problems related to interval graphs we know almost nothing in kernelization
complexity.  \pnamei{Interval Vertex Deletion} was recently shown to be
fixed-parameter tractable in single-exponential $10^k \cdot \poly(n)$ time~.


The parameterized complexity of \pnamei{Interval Deletion} is still wide
open.


For \pnamei{Interval Completion}, a subexponential time algorithm was
given~\cite{bliznets2014interval}, but this was famously achieved without a
polynomial kernel.  The kernelization complexity is a big open problem.


Hence, we know almost nothing about the kernelization complexity of interval
graphs.  Is \pnamei{Interval Editing} even \NP-hard? \fxnote{TODO check}



\paragraph{Proper interval graphs.}
\pnamei{Proper Interval Completion} admits a cubic
kernel~\cite{bessy2013polynomial} (contrast to the vertex deletion whose current
best kernel is contains $k^{53}$ vertices~\cite{fomin2013polynomial}).



\paragraph{$p$-leaf power graphs.}
The \emphi{$p$-leaf power graphs} are defined as follows.
\begin{definition}[$p$-leaf power]
  Let $T$ be a tree and $L_T$ be the leaves of $T$.  The $p$-leaf power of $T$
  is the graph $G = (L_T, E)$ where $uv \in E$ if and only if $\dist_T(u,v) \leq
  p$.
\end{definition}
It follows that the $1$-leaf power graphs are the independent sets\fxnote{TODO
  $K_2$ is a 1-leaf power of $K_2$} and the $2$-leaf power graphs are the
cluster graphs, the $P_3$-free graphs.  The editing, deletion and completion
problems towards $p$-leaf power graphs are \NP-hard for every $p \geq 3$.


\pnamei{$3$-Leaf Power Editing}, as well as the completion and deletion variant
all admit cubic vertex kernels~\cite{bessy2010polynomial}, where a graph is a
$3$-leaf power if it is a chordal bull-dart-gem-free graph (see
Section~\ref{sec:small-graphs} for small graphs).




\subsection{\fd}
\label{sec:kernel-intro:f-completion}

We here give a short survey on the history of polynomial kernels for \fd{} and
\fe{} for fixed $\mathcal{H}$ or $H$ (the case when $|\mathcal{H}| = 1$).  We
hope this motivates reasons for studying the kernelization complexity for these
problems further.


For a long time in parameterized complexity, the main focus of studies in \fd{}
was for the case when~$\F$ was an infinite family of graphs, e.g.,
\pname{Minimum Fill-in} or \pname{Interval
  Completion}~\cite{kaplan1999tractability, natanzon2000polynomial,
  villanger2009interval}.
% (The problem \pname{Minimum Fill-in} is also known as \pname{Minimum
% Triangulation} and \pname{Chordal Completion}, the problem of adding edges to
% obtain a chordal graph.)
This was mainly due to the fact that when~$\F$ is a finite family, \fd{} is
solvable on an $n$-vertex graph in time $f(k) \cdot n^{\bigO(1)}$ for some
function~$f$ by a simple branching argument; This was first observed by
Cai~\cite{cai1996fixedparameter}.  More precisely, if the maximum number of
non-edges in a graph from~$\F$ is~$d$, then the corresponding \fd{} is solvable
in time~$d^k \cdot n^{\bigO(1)}$.  The interest in \fd{} problems started to
increase with the advance of kernelization.  It appeared that from the
perspective of kernelization, even for the case of finite families~$\F$ the
problem is far from trivial.


\pause
%
Guo~\cite{guo2007problem} initiated the study of kernelization algorithms for
\fd{} in the case when the forbidden set~$\F$ contains the graph~$C_4$, see
Figure~\ref{fig:3graphs}.  (In fact, Guo considered edge deletion problems, but
they are polynomial time equivalent to completion problems to the complements of
the forbidden induced subgraphs.)  In the literature, the most studied graph
classes containing no induced~$C_4$ are the \emph{split graphs}, i.e., $\{2K_2,
C_4, C_5\}$-free graphs, \emph{threshold graphs}, i.e., $\{2K_2, P_4,
C_4\}$-free graphs, and $\{C_4, P_4\}$-free graphs, that is, \emph{trivially
  perfect graphs}~\cite{brandstadt1999graph}.
% citation also contained mahadev1995threshold
Guo obtained polynomial kernels for the completion problems for \emph{chain
  graphs}, split graphs, threshold graphs and trivially perfect graphs and
concluded that, as a consequence of his polynomial kernelization, the
corresponding \fd{} problems: \pname{Chain Completion}, \pname{Split
  Completion}, \pname{Threshold Completion} and \pname{Trivially Perfect
  Completion} are solvable in times $\bigO(2^k + mnk)$, $\bigO(5^k + m^4n)$,
$\bigO(4^k + kn^4)$, and $\bigO(4^k + kn^4)$, respectively.


\pause
%
Other known kernels before the upcoming work were
%
\pnamei{Triangle-Free Deletion}~\cite{brugmann2009generating},
%
\pnamei{Cluster Editing}~\cite{guo2009more,gramm2005graphmodeled},
%
\pnamei{Grid Editing}~\cite{diaz2006fast} (infinite obstruction set),
%
\pnamei{Biconnectivity Completion}~\cite{guo2010kernelization} (infinite
obstruction set),
%
\pnamei{Bridge-connectivity completion}~\cite{guo2010kernelization} (infinite
obstruction set).


Cai \footnote{Bodlaender, Cai, Chen, Fellows, Telle, Marx: Open Problems in
  Parameterized and Exact Computation—IWPEC 2006.  Utrecht University Technical
  Report UU-CS-2006-052 (2006)} raised the issue of determining the existence of
polynomial kernels for \pnamei{$H$-Free Edge Deletion} in IWPEC’06.

Later also Fellows, Langston, Rosamond and Shaw asked for \emph{linear} problem
kernels.

\pause
%
The work on kernelization of \fd{} problems was continued---nee took a change of
direction---by Kratsch and Wahlstr{\"o}m~\cite{kratsch2013two} who showed that
there exists a set $\F$ consisting of one graph on seven vertices for which
\fd{} does not admit a polynomial kernel.


Guillemot, Havet, Paul, Perez showed that \pnamei{$C_4$-Free Deletion}, or
\pnamei{$2K_2$-Free Completion} has no kernel, TODO~cite~Perez~thesis?

Guillemot et al.~\cite{guillemot2013nonexistence} showed that \pname{Cograph
  Completion}, i.e., the case $\F=\{ P_4\}$, admits a polynomial kernel, while
for $\F=\{ \overline{P_{\ell}}\}$, the complement of a path on $\ell$ vertices,
for $\ell \geq 7$, \fd{} has no polynomial kernel, as well as the
$\overline{C_\ell}$ for any $\ell \geq 4$.  \fxnote{todo fix story} These
results were significantly improved by Cai and
Cai~\cite{cai2015incompressibility}: For $\F = \{ P_\ell \}$ or $\F = \{ C_\ell
\}$, the problems \fd{} and \pname{$\F$-Edge Deletion} admit a polynomial kernel
if and only if the forbidden graph has at most three edges.


\pause
%
Then, even more kernels were shown.  Trivially Perfect Editing, Completion and
Deletion admit polynomial kernels by Drange and
Pilipczuk~\cite{drange2015polynomial} (see Chapter~\ref{cha:kernel-tp}), and
then also Chain and Threshold Editing, Completion and
Deletion~\cite{drange2015threshold} (see Chapter~\ref{cha:kernel-threshold}).


\subsection{Not \fd{} but almost}

A flip consensus tree, is, a bipartite graph $G = (V_c, V_t, E)$ where no
endpoint of an induced $P_5$ is a member of $V_t$.  In the problem
\pnamei{Minimum-Flip Consensus Tree}, we are given a bipartite\footnote{See
  Komusiewicz and Uhlmann~\cite{komusiewicz2014cubicvertex}} graph $G = (V_c,
V_t, E)$ and asked to flip at most $k$ edges to obtain a flip consensus tree.
The problem was shown to be \NP-complete by Chen et al., and later Böcker et
al.\ showed that the problem was solvable in time $O^{\star}(4.83^k)$, thus
being FPT.  Komusiewicz and Uhlmann~\cite{komusiewicz2014cubicvertex} showed
that the problem admitted a cubic vertex kernel.


\subsection{Exponential-sized kernels}
\label{sec:kernel-intro:exp-kernel}

\pnamei{Clique Cover}~\cite{gramm2006data} and \pnamei{Biclique
  Cover}~\cite{fleischner2007covering} --- ``they often provide the only known
way to show that a problem is fixed-parameter
tractable''~\cite{komusiewicz2014cubicvertex}.  Be that as it may.

\subsection{Open}
The kernelization complexity of these problems was asked in the survey by Liu,
Wang and Guo~\cite{liu2014overview}, together with several other interesting
questions.
\begin{itemize}
\item Improve problem kernel for \pnamei{Cograph Editing} to quadratic or linear
\item Improve problem kernel for \pnamei{$3$-Leaf Power} to quadratic or linear
\end{itemize}


==> summary.tex <==
\section{The Future}


We conclude by stating some open problems and some research questions for the
future. 

The results following Lewis and Yannakakis' work on the complexity of vertex
deletion problem~\cite{lewis1980nodedeletion} as well as Yannakakis' work on the
\pname{Minimum Fill-In} problem~\cite{yannakakis1981computing},
%
combined with Fomin and Villanger's proof that \pname{Minimum Fill-In} is
solvable in subexponential parameterized time~\cite{fomin2013subexponential},
%
have steadily been steered towards some new lines of research stated below.
%
Some of the main research questions following this thesis are:



\begin{itemize}
\item[$\star$] How far can we push subexponentiality beyond chordal graphs?
\item[$\star$] Which graph modification problems admit subexponential parameterized
  time algorithms?
\item[$\star$] Which graph modification problems admit polynomial kernels?
\end{itemize}





\subsection{Future directions}
\subsubsection{Complexity dichotomies for \HEC}
Can we come up with general classifications for~$\mathcal{H}$, possibly finite,
for which
\begin{itemize}
  % \item \HEC{} is \npci{} or in \cclass{P},
\item \HEC{} admits a polynomial kernel,
\item \HEC{} is solvable in subexponential parameterized time,
\end{itemize}
and similar questions for \HEE.
%
% Some results have recently started appearing.
% %
% In a series of preprints, Aravind, Sandeep, and Sivadasan announced that
% \pname{$H$-free Deletion}, \pname{Completion}, and \pname{Editing} is \npci{}
% if~$H$ is a graph with at least two edges, at least two non-edges, and at least
% three vertices, respectively~\cite{aravind2015parameterized,
%   aravind2015dichotomy}.  This is adding one step towards a better understanding
% of the complexity landscape of these problems.
%
%
For the question on kernelization, many results were achieved by
Cai~\cite{cai2012polynomial} in his Master thesis, which can be considered a
continuation of the work by Guillemot et al.~\cite{guillemot2013nonexistence}
and Kratsch and Wahlström~\cite{kratsch2013two}.
%
%
For the final question, however, absolutely no dichotomies or general theorems
are known except for the large classes of graphs we know do not have
subexponential parameterized time algorithms according to \ETH.  In the
aforementioned preprint by Aravind et al.~\cite{aravind2015parameterized}, they
do however show that for the problems mentioned there, a $2^{o(k)}\poly(n)$
lower bound under \ETH{} should follow.  Unfortunately, though, we are nowhere
near a broad understanding of this complexity landscape.




\subsubsection{Subexponentiality depends on kernelizability}
It seems, with the only \emph{possible} exception of \pname{Interval
  Completion}, that every graph modification problem solvable in subexponential
parameterized time admits a polynomial kernel.  Indeed, in many cases it is a
prerequisite for obtaining the algorithm.
%
Most subexponential parameterized time algorithms of this kind consists of
enumerating sublinear sized sets of vertices, however, to avoid getting
\cclass{XP}-type running times, the domain over which we enumerate must be of
size bounded polynomially in~$k$.
%
In the algorithm for \pname{Interval Completion}, the authors get away without
a polynomial kernel by only looking at small enough portions of the input graph
at the same time~\cite{bliznets2016subexponential}.

\index{trivially perfect graph}\index{cograph}\index{subexponential time
  algorithm}\index{polynomial kernel}


Since \pname{Cluster Deletion} admits a polynomial
kernel~\cite{chen2012kernel}, but does by the lower bounds result of Komusiewicz
and Uhlmann~\cite{komusiewicz2012cluster} not have a subexponential
parameterized time algorithm, the reverse direction does not hold.  It is also
easy to come up with problems for which there are subexponential parameterized
time algorithms, but no polynomial kernels, unless the polynomial hierarchy
collapses, but these problems are typically not \HEC s.  Consider the following
problem, which we slightly abusively call an \pname{Or-\HEC} problem:

\smallskip

% TODO add

%\defparproblem{OR-Trivially Perfect Completion}{$k$}
%% 
%{A graph~$G$ and an integer $k$}
%% 
%{Does~$G$ have a connected component~$C$ such that~$(C,k)$ is a yes-instance of
%  \pname{Trivially Perfect Completion}?}

\smallpause
%
This problem trivially cross-composes and is clearly \npci{}, so it cannot have
a polynomial kernel unless \ph.  Furthermore, running \pname{Trivially Perfect
  Completion} component-wise on the input graph~$G$ solves the problem in
subexponential parameterized time.






\subsubsection{The square root phenomenon: Chordal graphs}
All our results on subexponential parameterized time algorithms have been for
graph classes closely related to chordal graphs, that is, every graph class for
which modifying towards have been subclasses of chordal graphs.  There is a
minor exception in the case of pseudosplit graphs.  The pseudosplit graphs are
not chordal, however, they can be represented as split graphs, which are
chordal, plus~$n$ extra bits of information.



There is another exception in the problem \PBicE{}.
%
Recall that for a fixed~$p$, we can solve this problem in~$2^{O(\sqrt k \log k)}
+ \poly(n)$ time~\cite{DRS+15}.  However, this graph class is neither
chordal nor co-chordal since~$C_4$ is a bicluster and since~$2K_2 =
\overline{C_4}$ is a bicluster.
%
But, here the situation may still be salvaged by arguing that \PBicE{} is not
definable as an \HEE{} problem.  The graph class~$p$-bicluster---contrary to the
class of~$p$-cluster graphs---is not hereditary; removing the center vertex of a
$1$-starforest may result in a graph with arbitrarily many components.


So the interesting question is, for \HEE{} and \HEC{}, are
there~$\mathcal{H}$-free graph classes unrelated to chordal graphs for which any
of the two problems above are \npci{} and solvable in subexponential
parameterized time?
%
This question is also related to the third complexity dichotomy
for~$\mathcal{H}$; for which~$\mathcal{H}$ is \HEC{} and \HEE{} solvable in
subexponential parameterized time.

% \subsubsection{Some observations}
% In a recent paper on edge deletion problems, the authors conclude about
% subexponential parameterized time algorithms:
% \begin{quote}
%   Sometimes it may have an intuitive explanation, e.g., on chordal graphs,
%   destroying a hole needs a linear number of edge additions, but one single
%   edge deletion will suffice; however, we are not aware of such a simple
%   answer for the trivially perfect graphs~\cite{liu2015edge}.
% \end{quote}
% In fact, the same answer holds for completion versus deletion and editing on
% trivially perfect graphs; If we have a hole or a long path and we want to
% \emph{complete} to a trivially perfect graph, the optimal solution involves
% adding~$\Theta(n^2)$ edges, whereas if we want to delete (or similarly edit)
% to a trivially perfect graph, we simply delete every third edge, so~$O(n)$
% edges.  This means that in \TrivPC{}, the number of touched vertices
% is~$O(\sqrt k)$ when~$k$ is the budget, and in \TrivPD{} and \pname{Editing},
% the number of vertices touched is linear in the budget.

% This explanation, however, does not explain why \ThreshE, which on a long path
% and cycle will have a linear number of edited edges, admits a subexponential
% parameterized time algorithm.  However, if we take~$K_{n/2} \uplus K_{n/2}$,
% the graph consisting of two disjoint complete graphs, deleting to a threshold
% graph involves removing a quadratic number of edges, hence again touching
% only~$O(\sqrt k)$ vertices.





\subsubsection{Subexponential for targets with few components}
%
As we have discussed, Fomin et al.~\cite{fomin2014tight}, discovered that upon
bounding the number of connected components in the target graph by~$p$, they
could obtain subexponential time algorithms for the problem \pname{$p$-Cluster
  Editing}.  Such results are ruled out for \pname{Cluster Editing} under \ETH.
%
Misra et al.~\cite{misra2013subexponential} showed that this parameter does not
always help in the aim of obtaining subexponential time algorithm; it does not
for \pname{$p$-Club $d$-Cluster Editing}.
%
We saw that it \textit{does} help for \pname{Bicluster Editing}.  Allowing
arbitrarily many components in the target graph gives $2^{o(k)}\poly(n)$ lower
bounds under \ETH, whereas bounding this number gives $2^{O(p \sqrt{k}
  \log(pk))} + \poly(n)$ results.

Now, it is clear that bounding the number of components in the target for
trivially perfect graphs does not help; If a graph class is closed under adding
universal vertices, by adding a universal vertex to an input instance, any
optimal solution will always be connected.  An interesting question is to figure
out exactly when bounding the number of connected components in the solution
helps, and when not.






\subsection{Some concrete important open problems}


%
% CLASSIC NP
%
% % 17.2.1
% \subsubsection{Classical complexity}

% \begin{open}
%   What are sufficient and necessary conditions for \HED{} to be \NP-hard for
%   finite~$\mathcal{H}$?
% \end{open}

% \begin{open}
%   What are sufficient and necessary conditions for \HEE{} to be \NP-hard for
%   finite~$\mathcal{H}$?
% \end{open}
% %
% \smallpause
% %
% Here, we should always keep in mind that \pname{(Pseudo)Split Editing} is
% polynomial time solvable~\cite{hammer1981splittance}.

% \medpause
% %
% \begin{open}
%   Is \pname{Pseudosplit Editing} solvable in linear time?
% \end{open}
% \noindent
% %
% One place to start is to see whether one can read directly from the degree
% sequence the $C,S,I$-partitioning of the closest solution.



% % \bigpause
% % %
% % For fun we add the following problem.  Let \pname{Network Diversion} be the
% % following problem.  Given a graph~$G$, two vertices~$s$ and~$t$ as well as an
% % edge~$b$, and a budget~$k \in \mathbb{N}$.  Determine whether there is a set of
% % edges~$S$ such that in~$G-S$,~$b$ is a bridge between~$s$ and~$t$.  In other
% % words, determine the size of a minimum~$st$-cut containing~$b$.
% % \begin{open}
% %   Is \pname{Network Diversion} \NP-hard?
% % \end{open}





\subsubsection{Polynomial kernels}


\paragraph{Claw-free and line graphs.}
From the Master thesis of Cai~\cite{cai2012polynomial}, some of the interesting
remaining open questions are \HED{} for stars.
%
Denote by~$S_n$ the star on $n$ vertices, i.e., $K_{1,n-1}$.
%
\index{S03-free@$S_3$-free}\index{S04-free@$S_4$-free}%
\index{S11-free@$S_{11}$-free}\index{S07-free@$S_7$-free}%
%
It is well known that $S_3 = K_{1,2} = P_3$ does admit a $2k$ vertex kernel,
being the \pname{Cluster Deletion} problem.  On the other side,
Cai~\cite{cai2012polynomial} showed that \pname{$S_{11}$-free Deletion} does not
admit a polynomial kernel unless \ph.
%
\index{S11-free Deletion@\pname{$S_{11}$-free Deletion}}


Hence there is a large gap for~$H$ being~$S_4$, the claw, up to~$S_{10}$.
Closing this gap is an interesting theoretical question.  Recall that~$P_{\ell}$
and $C_{\ell}$ have the corresponding edge modification problems admitting
polynomial kernels if and only if the forbidden structure has at most three
edges.  Does the same hold for the stars?

\begin{open}
  Does \pname{claw-free Deletion} admit a polynomial kernel?
\end{open}

\smallskip\noindent
%
In a recent article, Cygan et al.~\cite{cygan2015polynomial} show, using an
overall strategy similar to what we did for \TrivPE, that deleting to
$\{\text{claw,diamond}\}$-free graphs admits a polynomial kernel.  This might
seem like an arbitrary graph class but is not; These are the line graphs of
triangle-free graphs~\cite{metelsky2003line,kratsch2012graph}.  This is also, as
they argue, a first important step towards deletion to claw-free graphs; They
highlight the next obstacle for obtaining a polynomial kernel ($X$ is here a
vertex modulator):
\begin{quote}
  Thus, we believe that for the sake of showing a polynomial kernel for
  \pname{claw-free Deletion}, one needs to understand the three special cases
  when $G-X$ is (a)~a line graph, (b)~a proper interval graph, and (c)~a
  co-bipartite graph. \cite{cygan2015polynomial}
\end{quote}

\noindent
%
Aravind and Sandeep~\cite{sandeep2015parameterized} improve the size of the
polynomial kernel of \pname{diamond-free Deletion} by
Cai~\cite{cai2012polynomial}, and ask
\begin{open}
  Does \pname{paw-free Deletion} admit a polynomial kernel?
\end{open}
%
\noindent
%
The paw is a claw plus an edge, and the diamond is a~$K_4$ minus an edge.
%
A graph $G$ is a paw-free graph if and only if each component of $G$ is
triangle-free or complete multipartite~\cite{olariu1988pawfree}.



An interesting first attempt to tighten the bound between $S_3$ and $S_{11}$
might be \pname{$S_7$-free Deletion}.
%
\index{S07-free Deletion@\pname{$S_{7}$-free Deletion}}
%
The reason why this might be interesting comes from considering the graph~$\KW$,
which is obtained from~$S_7$ by adding two non-incident edges.  The problem
$\KW$\pname{-free Deletion} does not admit a polynomial kernel unless
\ph~\cite{kratsch2013two}.
%
\index{HKW-free Deletion@$\KW$\pname{-free Deletion}}
%

\begin{open}
  Can we show that \pname{$S_7$-free Deletion} does not admit a polynomial
  kernel unless \ph?
\end{open}


\medpause
%
A graph class slightly related to claw-free graphs are the line graphs.
The class of \emph{line graph} is characterized by nine forbidden induced
subgraphs, the claw being one of them.

\begin{open}
  Does \pname{Line Deletion} admit a polynomial kernel?
\end{open}

\index{line graph}\index{claw-free graph}






\index{interval graph}

\paragraph{Interval graphs.}
%
The question of the parameterized complexity of \pname{Interval Completion} was
first asked in a FOCS paper in 1994 and then in a journal version by the same
authors, Kaplan, Shamir, and Tarjan in 1999~\cite{kaplan1999tractability}.  This
was answered in the positive more than a decade later by Villanger, Heggernes,
Paul, and Telle~\cite{villanger2009interval}.
%
In 2014, Bliznets, Fomin, Pilipczuk, and Pilipczuk showed that \pname{Interval
  Completion} is solvable in subexponential parameterized
time~\cite{bliznets2016subexponential}.
%
This is the first subexponential parameterized time algorithm for such a problem
given without relying on a polynomial kernelization.  To this date the
kernelization complexity of this problem is wide open.
%
\index{proper interval graph}\index{interval graph}

% Bliznets et al~\cite{bliznets2016subexponential} showed that \pname{Interval
% Completion} admits a subexponential parameterized time algorithm.  They did
% however not have a polynomial kernel, and had to walk around that issue.  The
% following question is a highly interesting question, especially with respect
% to the question below of whether subexponentiality and polynomial
% kernelizability are somehow related in these types of problems:

\begin{open}
  Does \pname{Interval Completion} admit a polynomial kernel.
\end{open}



\bigskip
\noindent
%
There is currently a large gap in our knowledge of \ChordE{}.
%
The problem was just recently proved to be \FPT{} by Cao and
Marx~\cite{cao2014chordal}, but they give a~$k^k$-type algorithm.
%
There is a lower bound of the type $2^{o(\sqrt k)} \cdot \poly(n)$ using \ETH.
%
There is a big gap between
\[
2^{O(k \log k)}\poly(n) \text{ and }2^{o(\sqrt k)} \poly(n).
\]
\noindent
%
What is the correct bound?  Is it $2^{\Theta(k)}\poly(n)$?
%
In addition to the question in light of the optimality programme question, there
is a question of whether the problem admits a polynomial kernel.

\begin{open}
  Does \ChordE{} admit a polynomial kernel?
\end{open}


\medpause
%
Finally, the following problem is still a valid and interesting problem, despite
that we know that the problems have \corp{}
kernels~\cite{kratsch2014compression}.
%
Providing randomized kernels demanded completely new tools for these problems,
namely applying matroid theory for preprocessing.  This has already sparked new
research directions, and there is a hope that the same thing may happen for the
deterministic version.

\index{bipartite graph}
%
\begin{open}
  Do \pname{Odd Cycle Transversal} and \pname{Edge Bipartization} admit
  deterministic polynomial kernels?
\end{open}








\subsubsection{Subexponential time}

Of all the \HEC{} problems we know to be solvable in subexponential
parameterized time, only one is known to be solvable in time $2^{O(\sqrt k)}
\poly(n)$: \SplitC{}~\cite{cygan2015parameterized}.
%
In addition, only one is not known to be solvable in time $2^{\osl}\poly(n)$,
namely \pname{Proper Interval Completion}.  A natural next step in the
optimality programme is to improve the $2^{O(k^{2/3} \log k)} + \poly(n)$
algorithm by Bliznets et al.~\cite{bliznets2015subexponential} to an algorithm
running in time $2^{\osl} \poly(n)$.
%
In light of the optimality programme and the few lower bounds we have for these
graph problems, a most interesting question is ``what are the correct running
times?''

\index{chordal graph}\index{subexponential parameterized time algorithm}

As stated above, Fomin and Villanger~\cite{fomin2013subexponential} noticed that
under \ETH, we cannot solve \ChordC{} in time $2^{O(k^{1/6})}\poly(n)$.
%
Bliznets et al.\ recently improved this to a lower bound on the form
\[
2^{O(k^{1/4} / \log^c k)} \cdot \poly(n) ,
\]
for some integer~$c$, simultaneously providing lower bounds for the problems
\pname{Interval Completion}, \pname{Proper Interval Completion},
\pname{Threshold Completion}, \pname{Chain Completion}, and \pname{Trivially
  Perfect Completion}~\cite{bliznets2016lower}.
%
Under the assumption that there is no subexponential-time approximation scheme
for \pname{Min Bisection} on $d$-regular graphs, they give stronger bounds of
the form $2^{o(\sqrt k)} \poly(n)$ for all of those problems as well.

\begin{open}
  Is \pname{Chordal Completion} solvable in $2^{O(\sqrt k)} \cdot \poly(n)$
  time?
\end{open}




\begin{open}
  Does there exist a set~$\mathcal{H}$ such that \HEC{} is solvable in $2^{o(k)}
  \cdot \poly(n)$ but does not admit a polynomial kernel?
\end{open}

\noindent
%
Recall from above that there are plenty of problems that are solvable in
subexponential parameterized time but does not admit a polynomial
kernel---trivially cross composable problems like
\pname{Planar~$k$-path}~\cite{demaine2005subexponential,
  bodlaender2009problems}, or any problem of the form ``does the input graph
have a connected component~$C$ which is lacking~$k$ edges from being, say, a
chordal graph?''





\paragraph{Going beyond chordal graphs.}
%
%
% \pname{Circular Arc Graph Editing} solvable in \FPT{} time?
%
% 
The \emph{threshold signed} graphs are exactly the graphs of dilworth number 2,
whereas threshold graphs are graphs of dilworth number 1.
%
It is the first next level of natural generalizations of threshold graphs.  The
definition is the following:
\begin{definition}[Threshold signed graph]
  A graph is a \emph{threshold signed} graph if there are two positive reals~$s
  \in \mathbb{R}$ and~$t \in \mathbb{R}$ and a weight function~$w: V \to
  \mathbb{R}$, such that for every vertex~$v$,~$w(v) \leq \min\{s,t\}$ and for
  every two vertices~$u,v$,~$uv \in E(G)$ if and only if~$|w(u) + w(v) | \geq s$
  or~$|w(u) - w(v)| \geq t$.
\end{definition}

\begin{open}
  Is \pname{Threshold Signed Completion} \FPT?  Is it solvable in
  subexponential parameterized time?
\end{open}




\index{permutation graph}

\noindent
%
The permutation graphs are a superclass of the threshold signed graphs, and are
best definable using a geometric intersection model, like the interval graphs.
\begin{definition}[Permutation graph]
  A graph is a permutation graph if and only if it has an intersection model
  consisting of straight lines between two parallel
  lines~\cite{brandstadt1999graph}.
\end{definition}

\begin{open}
  Is \pname{Permutation Completion} \FPT?  Is it solvable in subexponential
  parameterized time?
\end{open}



\noindent
% % 
% The following definitions are equivalent:
% \begin{itemize}
A graph is a circle-polygon graph if it is the intersection graph of convex
polygons inscribed in a circle.
% \item A graph is a circle-polygon graph if there exists a bijection from
%   vertices to sets of connected non-intersecting chords inscribed in a circle
%   such that two vertices are adjacent iff their sets contains at least one pair
%   of intersecting chords.
% \end{itemize}

% \noindent
% % 
\begin{open}
  Is \pname{circle-polygon Completion} \FPT{}? Is it solvable in subexponential
  parameterized time?
\end{open}


% A circle-polygon graph is also referred to as a spider graph
% \begin{definition}[Spider graph]
%   A graph is is a spider graph if every vertex~$v_i$ can be assigned a set~$S_i$
%   of points on the circle such that~$v_i$ and~$v_j$ are adjacent if and only if
%   there exist~$a,b \in S_i$ and~$x,y \in S_j$ such that $a<x<b<y$ or $x<a<y<b$.
% \end{definition}


% A bridged graph is a graph whose every cycle of length at least 4 has a
% bridge, a bridge of a cycle being a shortest path connecting to
% non-consecutive vertices of the cycle.  Is Bridged Completion NP-complete?
% SUBEPT?


\subsection{Local search}

Mention very recent survey of Nidermeier et al.\ on arxiv.






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "survey"
%%% End:

